Individual Welfare Guarantees in the Autobidding World with Machine-learned Advice

Online advertising channels have commonly focused on maximizing total advertiser value (or welfare) to enhance long-run retention and channel healthiness. Previous literature has studied auction design by incorporating machine learning predictions on advertiser values (also known as machine-learned advice) through various forms to improve total welfare. Yet, such improvements could come at the cost of individual bidders' welfare and do not shed light on how particular advertiser bidding strategies impact welfare. Motivated by this, we present an analysis on an individual bidder's welfare loss in the autobidding world for auctions with and without machine-learned advice, and also uncover how advertiser strategies relate to such losses. In particular, we demonstrate how ad platforms can utilize ML advice to improve welfare guarantee on the aggregate and individual bidder level by setting ML advice as personalized reserve prices when the platform consists of autobidders who maximize value while respecting a return-on-ad spent (ROAS) constraint. Under parallel VCG auctions with such ML advice-based reserves, we present a worst-case welfare lower-bound guarantee for an individual autobidder, and show that the lower-bound guarantee is positively correlated with ML advice quality as well the scale of bids induced by the autobidder's bidding strategies. Further, we prove an impossibility result showing that no truthful, and possibly randomized mechanism with anonymous allocations can achieve universally better individual welfare guarantees than VCG, in presence of personalized reserves based on ML-advice of equal quality. Moreover, we extend our individual welfare guarantee results to generalized first price (GFP) and generalized second price (GSP) auctions.

==> 00_extendedabstract.tex <==

Online advertising channels  have commonly focused on maximizing total advertiser value (or welfare) to enhance long-run retention and channel healthiness. Previous literature has studied auction design by incorporating machine learning predictions on advertiser values (also known as \textit{machine-learned advice}) through various forms to improve total welfare. Yet, such improvements could come at the cost of individual bidders' welfare and do not shed light on how particular advertiser bidding strategies impact welfare.

Motivated by this, we present an analysis on an individual bidder's welfare loss in the autobidding world for auctions with and without machine-learned advice, and also uncover how advertiser strategies relate to such losses. In particular, we demonstrate how ad platforms can utilize ML advice to improve welfare guarantee on the aggregate and individual bidder level by setting ML advice as personalized reserve prices when the platform consists of \textit{autobidders} who maximize value while respecting a return-on-ad spent (ROAS) constraint. Under parallel VCG auctions with such  ML advice-based reserves, we present a worst-case welfare lower-bound guarantee for an individual autobidder, and show that the lower-bound guarantee is positively correlated with ML advice quality as well the scale of bids induced by the autobidder's bidding strategies. Further, we prove an impossibility result showing that no truthful, and possibly randomized mechanism with anonymous allocations can achieve universally better individual welfare guarantees than VCG, in presence of personalized reserves based on ML-advice of  equal quality. Moreover, we extend our individual welfare guarantee results to generalized first price (GFP)  and generalized second price (GSP) auctions. Finally, we present numerical studies using semi-synthetic data derived from ad auction logs of a major search ad platform to showcase improvements in individual welfare when setting personalized reserve prices with ML-advice.

==> Add_pricing.tex <==
This appendix is a complete version of our discussions in Section \ref{sec:shortenedpricing}. 

Here, we take the alternative perspective of the seller and consider the pricing problem against a single  ROI and budget constrained buyer. {We view studying the single buyer scenario as a first step for future research on pricing against multiple budget and ROI constrained buyers. We also remark that pricing to a single buyer allows the buyer to more easily manipulate the seller's algorithms, and hence is of theoretical interest to understand whether the seller can harness this manipulative power. The single buyer pricing problem has also been studied in \cite{kleinberg2003value,amin2013learning,braverman2018selling}.}

In this single buyer scenario, the second price auction effectively becomes a posted price auction, where the seller's price takes the role of highest competing bid value $d_{t}$. More specifically, the buyer
still decides on some bid value $b_{t}$, but instead of having the buyer actually submit the bid, the buyer decides to take the item at period $t$ and pay price $d_{t}$  if 
$b_{t} \geq d_{t}$, or leave the item and pay nothing otherwise. That being said, any bidding strategy (e.g. $\textsc{CTBR}_{\algo}$) for the second price auction can be effectively transformed into a ``take or leave'' strategy for the posted price auction.
%In light of this view, the seller's posted price can be thought of as the highest competing price to the buyer, which is exactly the buyer's payment if her bid is greater than the highest competing bid as in the second price auction.
We note that the seller does not get to observe the buyer's ``bid'' but instead only knows whether the buyer took the item or not. %Also, the buyer observes both $v_{t}$ and $d_{t}$ before making a take/leave decision.




\textbf{Seller's pricing problem.}
Consider the seller committing to a finite price set $\mathcal{D} = \{D^{m}\}_{m\in[M]}$ where $D^{1} > \dots > D^{M}$. The seller sets a price $d_{t} \in \mathcal{D}$ during each period against a \textit{value-maximizing} buyer (whose capital cost $\alpha = 0$). \footnote{In the posted price setting, assuming the buyer's capital cost $\alpha =0$ is without loss of generality. This is because before the buyer makes a take/leave decision, she gets to observe both her valuation $v_{t}$ and price $d_{t}$. Hence, in the buyer's hindsight problem $\opt(\left\{v_{t},d_{t}\right\}_{t\in [T]};\alpha,\gamma,\rho)$ defined in Equation (\ref{eq:defOpt}), the buyer can rescale her valuations by setting $\widetilde{v}_{t} = v_{t} - \alpha d_{t}$ as well as her target ROI $\widetilde{\gamma}= \gamma - \alpha$. This will result in the equivalent hindsight problem 
$\widetilde{\opt}(\left\{\widetilde{v}_{t},d_{t}\right\}_{t\in [T]};0, \widetilde{\gamma},\rho) \defeq \max_{\bm{z} \in [0,1]^{T}}  \sum_{t\in[T]} \widetilde{v}_{t}z_{t} \quad
\textrm{s.t.} \sum_{t\in [T]} \left(\widetilde{v}_{t} - \widetilde{\gamma} d_{t}\right)z_{t}\geq 0,~ \sum_{t\in [T]}  d_{t}z_{t}\leq \rho T$, which implies that we can simply assume $\alpha =0$. }
Then, the buyer observes both $d_{t}$ and its valuation $v_{t} $ and makes a take/leave decision $z_{t}\in \{0,1\}$ based on some learning algorithm that satisfies both ROI and budget constraint in Equation (\ref{eq:feasiblestrat}). Here, we assume that the buyer's valuations are supported on the set $\mathcal{\V} = \{\V^{n}\}_{n\in[N]}$ where $\V^{1} > \dots > \V^{N}$ and associated with some probability distribution $\valp \in \Delta_{N}$ such that $\prob(v_{t} = \V^{n}) = \valpe^{n}$ for any period $t \in [T]$. On a separate note, $ \{D^{m}\}_{m\in[M]}$ and $\{\V^{n}\}_{n\in[N]}$
can be thought of as the unique values of highest competing bids and valuations in the set $\mathcal{W} = \{(v^{k},d^{k})\}_{k \in [K]}$ of the previous sections, i.e. $\mathcal{W} = \mathcal{V}  \times  \mathcal{D}$, where $K = MN$. Furthermore, imposing any distribution $\widetilde{\valp}\in \Delta_{M}$ on support $\mathcal{D}$, combined with distribution $\valp$ on $\mathcal{\V}$, induces a product distribution $\bm{p} =\valp \times \widetilde{\valp}$ over
$\mathcal{W} $.

The buyer's target ROI $\gamma$ and budget rate $\rho$ are private to the buyer and is unknown to the seller. Both the seller and the buyer do not know the valuation distribution $\valp$, and hence learn how to price and make take/leave decisions respectively as time proceeds. In other words,
the posted price auction involves \emph{a two-sided learning paradigm} where both the seller and buyer adopt different online decision-making strategies that interact with one another. {Our goal is to better understand whether we can design an effective pricing algorithm facing an environment that is driven by the buyer's unknown algorithm. }

\textbf{Seller's regret.}
We evaluate the performance of any sequence of pricing decision $\{d_{t}\}_{t \in [T]} \in \mathcal{D}^{T}$ by benchmarking its realized revenue, namely $\sum_{t\in[T]}d_{t}z_{t}$, to the maximum revenue that could have been obtained if the seller had set a fixed price over all $T$ periods assuming the buyer makes optimal decisions. Mathematically,  we first rewrite the buyer's problem in Equation (\ref{eq:reformOPT}) as followed for any fixed seller price  $d \in \mathcal{D}$ as
\begin{align}
\label{eq:pricing:buyerutil}
\util(d) = \max_{\bm{x}\in [0,1]^{N}}  \sum_{n\in[N]} \valpe^{n}\V^{n} x^{n} 
\quad \textrm{s.t.} \sum_{n\in[N]} \valpe^{n}\left(\V^{n} - \gamma d\right)x^{n}\geq 0,\text{ and }
 d\sum_{n\in[N]} \valpe^{n} x^{n}\leq \rho \,.
\end{align}
In light of Theorem  \ref{lem:thresholdOptSol}, we let $\bm{x}_{d} \in [0,1]^{N}$ be the unique optimal threshold solution to $\util(d)$ for any $d \in \mathcal{D}$, and note that the optimal solution induces a per-period expenditure of
\begin{align} \label{eq:revenue}
\rev(d) \defeq d\sum_{n\in [N]} \valpe^{n} x_{d}^{n}\,,
\end{align}
which is also the expected per-period revenue of the seller when the buyer knows $ \valp$ and acts optimally. We will refer to $\rev(\cdot)$ as the seller's \textit{revenue function}. Here, we remark that $\sum_{n\in [N]} \valpe^{n} x_{d}^{n}$ is the probability that the buyer decides to take price $d$. Then, for any sequence of pricing decisions
$\{d_{t}\}_{t \in [T]} \in \mathcal{D}^{T}$, we define the seller's regret over $T$ periods to be
\begin{align}
   \text{Reg}_{\text{sell}} = T\max_{d\in \mathcal{D}}\rev(d) - \sum_{t\in [T]}\E\left[d_{t}z_{t}\right]\,,
\end{align}
where the expectation is taken w.r.t. $\{(v_{t},d_{t})\}$ and randomness in the buyer's strategy.


The benchmark $\util(d)$ is in fact equivalent to our definition of $\util(\bm{p};0,\gamma,\rho)$ in Section \ref{sec:reform}. Assume the seller sets price $d_{t} = \D^{m}\in \mathcal{D}$ for some $m \in [M]$ and
for all $t \in [T]$. In this case the buyer's hindsight benchmark is given by $\opt(\left\{v_{t},D^{m}\right\}_{t\in [T]};0,\gamma,\rho)$. Under this fixed price scenario, $d_{t} $ can be viewed as being drawn from the distribution $\bm{e}^{m} \in \Delta_{M}$ ($m$'th unit vector in $\R^{M}$), which then induces the product distribution $\bm{p} = \valp \times \bm{e}^{m}\in\Delta_{K}$ over $\mathcal{W}$. Then, it is not difficult to see for any $m\in[M]$,  $\util(\D^{m})$ is equivalent to $\util(\valp \times \bm{e}^{m};0,\gamma,\rho)$.\footnote{Consider any decision vector  $\widetilde{\bm{x}} \in [0,1]^{K}$ that is feasible to $\util(\valp \times \bm{e}^{m};0,\gamma,\rho)$. Using the definition that
$\bm{p} = \valp \times \bm{e}^{m}$, we have
$p^{k}  =g^{n} $ is $(v^{k},d^{k}) = (\V^{n},\D^{m})$ and $p^{k}  =0$ otherwise. 
% $p^{k} = \begin{cases}g^{n} & \text{if } (v^{k},d^{k}) = (\V^{n},\D^{m})\\ 0 & \text{otherwise}\end{cases}$.
Thus, the objective of $\util(\valp \times \bm{e}^{m};0,\gamma,\rho)$, namely $\sum_{k \in [K]}p^{k} v^{k} \widetilde{x}^{k} = \sum_{n \in [N]} \sum_{k:v^{k} = \V^{N}}p^{k} v^{k} \widetilde{x}^{k} =\sum_{n \in [N]}g^{n}\V^{n}x^{n} $ where $x^{n}$ is the change of variable for $\widetilde{x}^{k}$ when $k\in[N]$ satisfies $ (v^{k},d^{k}) = (\V^{n},\D^{m})$. A similar argument shows that the two constraints are also equivalent, i.e.
$\sum_{k \in [K]}p^{k} d^{k} \widetilde{x}^{k} =  D^{m}\sum_{n\in[N]} \valpe^{n} x^{n}$ and $\sum_{k \in [K]}p^{k} \left(v^{k} - \gamma d^{k}\right) \widetilde{x}^{k} = \sum_{n\in[N]} \valpe^{n}\left(\V^{n} - \gamma D^{m}\right)x^{n}$.}
This equivalency between $\util(d)$ and $\util(\bm{p};0,\gamma,\rho)$ suggests that the benchmark $\util(d)$ indeed implies optimal buyer actions, as for any $m\in [M]$ such that $D^{m} \in \mathcal{D}$, we have $\util(D^{m}) =\util(\valp \times \bm{e}^{m};0,\gamma,\rho) \geq \E\left[\opt(\left\{v_{t},D^{m}\right\}_{t\in [T]};0,\gamma,\rho)\right]$, where the final inequality follows from Theorem \ref{thm:optbidding}.



 Finally, we remark the seller's regret resembles that of an $M$-arm multi-arm bandit (MAB) problem (see \cite{lattimore2020bandit} for a detailed introduction), where we can view each price $D^{m} \in \mathcal{D}$ as an arm and $D^{m}z_{t}$ to be the reward by pulling arm $m$. Nevertheless, we point out that our problem is more complex as the seller's reward $D^{m}z_{t}$ for setting price $D^{m}$ during period $t$ is related to the buyer-specific algorithm, which likely depends on the buyer's past decisions as well as past prices set by the seller. Although our pricing problem is more difficult than MAB which typically requires the decision maker to explore all $M$ arms, in the next section we demonstrate that by exploiting the special structures of our problem, we only need to explore $\mathcal{O}(\log(M))$ arms (prices).





\subsection{Bell-shaped Structure of the Revenue Function}
In this section, we first motivate our pricing algorithm by analyzing some underlying  structures of the seller revenue $\rev(d)$ defined in Equation (\ref{eq:revenue}). The goal of this section is to develop efficient ways to identify $\arg\max_{d\in\mathcal{D}}\rev(d)$ by avoiding exploring each possible price in $\mathcal{D}$ which will result in a regret that scales linearly in the number of prices $M$. In the rest of the paper, we make the following assumption to rule out trivial problem instances (e.g. cases when the optimal solution $\bm{x}_{d}$ corresponding to some $d\in \mathcal {D}$ has all 0 entries or when one of the constraints are redundant):
\begin{assumption}
\label{assum:price:nontriv}
For any $d \in \mathcal{D}$, assume $V^{N} - \gamma d < 0$, $\V^{1} - \gamma d > 0$ and $\sum_{n \in [N]}(\V^{n} - \gamma d)\valpe^{n} \neq 0$. Furthermore, assume $\Bar{d} > \rho$ and  $\underline{d} < \rho$.
\end{assumption}

%\jason{I simplified the following definitions, and it should be very intuitive. I think having these definitions better convey my message regarding the bell-shaped revenue curve.}
 To begin with, we  categorize all prices  $d\in \mathcal{D}$ according to whether constraints are binding under the corresponding optimal solution $\bm{x}_{d}$. 
\begin{definition}Fix target ROI $\gamma $, budget rate $\rho$, valuation distribution $\valp\in \Delta_{K}$ and selling price $d \in \mathcal{D}$. Recall $\bm{x}_{d}$ is the optimal threshold-based solution to $\util(d)$ in Equation (\ref{eq:pricing:buyerutil}). Then we say $d$ is
\begin{itemize}
    \item \textbf{Non-binding}, if under $\bm{x}_{d}$, both constraints are non binding, i.e., $d\sum_{n \in [N]}\valpe^{n}x_{d}^{n} < \rho$ and 
    $\sum_{n\in[N]}\left(\V^{n} - \gamma d\right)\valpe^{n}x_{d}^{n} > 0$;
    \item \textbf{Budget binding} if under $\bm{x}_{d}$, the budget constraints is binding, i.e.
    $d\sum_{n \in [N]}\valpe^{n}x_{d}^{n} = \rho$ and $\sum_{n \in [N]}(\V^{n} - \gamma d)\valpe^{n}x_{d}^{n}\geq 0$;
    \item \textbf{ROI binding}  if under $\bm{x}_{d}$, the ROI constraint is binding, i.e. $\sum_{n \in [N]}(\V^{k} - \gamma d)\valpe^{n}x_{d}^{n} = 0$ and $d\sum_{n \in [N]}\valpe^{n}x_{d}^{n}\leq \rho$.
\end{itemize}
\end{definition}
It is apparent that any price $d\in \mathcal{D}$ must belong to at least one of these categories. Also, if a price is non-binding, it cannot be budget binding or ROI binding. However, it may be possible that a price $d$ is both budget binding and ROI binding.  This can only occur for certain model primitives $\rho, \gamma, \valp$. We also point out  that for any budget binding price $d \in \mathcal{D}$, the seller would like to extract the entire budget from the buyer since the per-period revenue under optimal buyer action is $\rev(d) = d\sum_{n \in [N]}\valpe^{n}x_{d}^{n}= \rho$.
% \begin{lemma}
% \label{eq:phaseopt}
% If $d \in \mathcal{D}_{\nb}$ is non-binding, then the optimal solution 
% $\bm{x}_{d}$ to $\util(d)$ is given by $\bm{x}_{d} =\sum_{k\in[\kappa_{\alpha}]} \bm{e}^{k}$. If $d \in \mathcal{D}_{\budb}$ is budget binding, then  $\bm{x}_{d} = \min\left\{\bm{x}_{d}^{\bud}, \sum_{k\in[\kappa_{\alpha}]} \bm{e}^{k} \right\}$.  If $d \in \mathcal{D}_{\roib}$ is ROI binding, then $\bm{x}_{d} = \min\left\{\bm{x}_{d}^{\ROI}, \sum_{k\in[\kappa_{\alpha}]} \bm{e}^{k} \right\}$.
% \end{lemma}

Our main result of this subsection is the following Theorem \ref{thm:pricing:optd}, which states that as we traverse $\mathcal{D}$ in increasing price order, prices are first non-binding and the revenue $\rev(d)$ increases in $d$; then prices become budget binding, where revenue remains constant at $\rev(d) = \rho$; finally prices become ROI binding, where $\rev(d)$ decreases in $d$. The proof can be found in Appendix \ref{proof:thm:pricing:optd}.

\begin{theorem}[Bell-shaped Structure of the Revenue Function]
\label{thm:pricing:optd}
Suppose that Assumption $\ref{assum:price:nontriv}$ holds. Then, the following hold  
\begin{enumerate}
    \item For any non-binding prices $d,\widetilde{d}$, if $d< \widetilde{d}$ then $\rev(d) < \rev(\widetilde{d})$. 
    \item If $d$ is budget binding, any price $\widetilde{d} > d$ cannot be non-binding, which means $\widetilde{d}$ is budget binding or ROI binding.
    \item If $d$ is ROI binding, then any $\widetilde{d} > d$  must also be ROI binding. Furthermore, $\rev(d) > \rev(\widetilde{d})$. 
\end{enumerate}
\end{theorem}
We provide an illustration of Theorem \ref{thm:pricing:optd} in Figure \ref{fig:transition} that depicts the ``non-binding $\rightarrow$ budget binding $\rightarrow$ ROI binding''  transition phenomenon, as well as a corresponding revenue ``increase $\rightarrow$ plateau $\rightarrow$ decrease'', as we traverse prices in increasing order. We note that for specific model primitives $\valp ,\gamma, \rho$, there may exists no budget binding prices
(as shown in right subfigure in Figure \ref{fig:transition}), meaning that there are scenarios in which it is impossible for the buyer to extract the entire buyer budget. Nevertheless, this transition phenomena suggests that we can efficiently identify the maximizing revenue $\arg\max_{d\in\mathcal{D}}\rev(d)$ by utilizing a simple binary search approach. Hence, we utilize this structure of $\rev(d)$ to motivate our pricing algorithm. 


\subsection{Pricing Algorithm against an ROI and Budget Constrained Buyer}





The main challenge the seller faces is her lack of knowledge on the buyer's model primitives, namely the buyer's valuation distribution $\valp$, target ROI $\gamma$ and budget rate $\rho$. Furthermore, the seller has limited information feedback as she only observes whether the buyer took the price or not, i.e., the seller only observes the outcome $z_{t} \in \{0,1\}$. This lack of information makes it very difficult for the seller to estimate the buyer's model primitives. Nevertheless, we propose a simple pricing algorithm that bypasses this lack of knowledge via exploiting the price transition phenomenon as characterized in Theorem \ref{thm:pricing:optd} and Figure \ref{fig:transition}. We demonstrate that this algorithm achieves good performance when facing a general class of algorithms that is adaptive to nonstationary environments.
\begin{figure}[!ht]
\includegraphics[width=12cm]{trans.png}
\centering
\caption{\footnotesize \textbf{Seller revenue function bell-shape structure.} Model primitives: number of unique buyer valuations $N = 6$, valuation set $\mathcal{V} = (0.6,0.5,0.4,0.3,0.2,0.1)$, valuation distribution $\valp = (0.1,0.1,0.2,0.1,0.2,0.3)$, number of unique selling prices $M = 21$, seller price set $\mathcal{D} = (0.5,0.48 \dots 0.1)$, buyer budget rate $\rho = 0.2$, capital cost $\alpha = 0$. The left and right subfigures correspond to target ROI $\gamma = 1.3$ and $1.7$ respectively. In both cases, prices transition from non-binding to budget binding, and finally to ROI binnding. Revenue $\rev(d)$ increases as in $d$ when prices are non-binding, decreases in $d$ when prices are ROI binding, and remains at $\rho$ when prices are budget binding. Note that when $\gamma = 1.7$, there are no budget binding prices.}  
\label{fig:transition}
\end{figure}


Our proposed pricing algorithm consists of an exploration phase and an exploitation phase.  During the exploration phase, the algorithm searches for a revenue maximizing price $D^{*} \in \arg\max_{d\in \mathcal{D}}\rev(d)$ through an episodic structure: the seller initiates the first episode  $\mathcal{E}_{1}$, and fixes the price chosen in this episode $D_{1}$ for $E$ consecutive periods. At the end of the episode (i.e. after $E$ periods since the beginning of the episode), the seller records the average per-period revenue $\Hat{\rev}(D_{1}) = \frac{D_{1}}{E}\sum_{t\in \mathcal{E}_{1}}z_{t}$, where $z_{t} \in \{0,1\}$ indicates whether the buyer takes the price at time $t \in \mathcal{E}_{1}$. The process then repeats as the seller moves on to episodes $\mathcal{E}_{2}, \dots $ This exploration phase eventually terminates when the seller has explored enough prices.
The seller's pricing decision in each episode is governed by a binary search procedure over the set $\mathcal{D}$, such that
every price is chosen at most once across all episodes, and the exploration phase will have $\mathcal{O}(\log(M))$ episodes. Our pricing algorithm is detailed in 
Algorithm \ref{alg:pricing}. 

We note that our proposed algorithm does not try to learn the buyer's model primitives.
We further point out that 
such a binary-search approach is a natural choice to identify revenue-optimal prices in the simplest monopolistic pricing setting under a typical unimodal 
assumption, \footnote{In monopolistic pricing, the revenue-optimal price $p^{*}$ is charachterized by $p^{*}  = \arg\max_{p} pF(p)$, where $F$ is the cdf of buyer valuations. A typical assumption is such that the function $pF(p)$ is unimodal.} and one may wonder whether this approach can have good performances against a much more complex setting where the buyer is ROI and budget constrained and aims to learn her optimal bidding strategy. Surprisingly, in the next section we are in fact able to show this simple approach achieves good performances against buyers who are adaptive to price changes. 


\begin{algorithm}[H]
    \centering
    \caption{Binary Search Exploration Exploitation}\label{alg:pricing}
    \footnotesize
    \begin{algorithmic}[1]
    \Require Episode length $E$.
    \State Initialize iteration index $\iter= 1$.
    \State  {\textbf{[Exploration]}}:
    \State Set $\D^{1}$ for $E$ consecutive periods, and record per-period revenue $\Hat{\rev}\left(D^{1}\right)$. Then 
	set $\D^{M}$ for $E$ consecutive periods, and record per-period revenue $\Hat{\rev}\left(D^{M}\right)$.
	\State Set $\term\leftarrow \arg\max_{m\in \{1,M\}} \Hat{\rev}\left(\D^{m}\right)$\; 
	$\lef= 1$, $\rig = M$, $\med = \lfloor\frac{\lef+\rig}{2}\rfloor$.
	\While{$\lef < \rig$}
	\State $\iter \leftarrow \iter+1$.
	\If{per-period revenue $\Hat{\rev}\left(\D^{k}\right)$ is not recorded for $k = \med,\med+1$}
	\State{Set
		price $\D^{k}$ for $E$ consecutive periods and record per-period revenue $\Hat{\rev}\left(\D^{k}\right)$ for $k = \med, \med+1$}
	 \EndIf
	 \If{$\Hat{\rev}\left(\D^{\med}\right)  < \Hat{\rev}\left(\D^{\med+1}\right)$} 
	 \State{Set $\term\leftarrow \arg\max_{m\in \{\term,\med+1\}} \Hat{\rev}\left(\D^{m}\right)$, $\lef \leftarrow \med+1$, $\med \leftarrow \lfloor\frac{\lef+\rig}{2}\rfloor$}
	 \Else 
	 \State Set $\term\leftarrow \arg\max_{m\in \{\term,\med\}} \Hat{\rev}\left(\D^{m}\right)$, $\rig \leftarrow \med-1$, $\med \leftarrow \lfloor\frac{\lef+\rig}{2}\rfloor$
	 \EndIf
	\EndWhile
	\State {\textbf{[Exploitation]}: Set price $\D^{\term}$ for the remaining periods.}
    \end{algorithmic}
\end{algorithm}



\subsection{Regret Analysis of Our Pricing Algorithm}
In this section, we provide theoretical guarantees for our proposed pricing algorithm against a class of buyer's bidding strategies.
Recall that the seller is pricing against a buyer who is subject to both budget and ROI constraints, and adopts some algorithm that satisfies both ROI and budget constraint in Equation (\ref{eq:feasiblestrat}) to maximize total cumulative value.
 The class of strategies that we consider imposes some notion of adaptiveness to non-stationary environments, as discussed in the following definition.% \ref{def:robust}.
%\jason{I am not super satisfied with this definition. Please let me know what you think. }
\begin{definition}[ $\xi$-Adaptive  Bidding Strategies]
\label{def:robust}
Assume the $T$-period horizon is divided into $H$ consecutive episodes $\mathcal{E}_{1} \dots \mathcal{E}_{H}$, i.e.$\sum_{h\in[H]}|\mathcal{E}_{h}| = T$. In each episode $h \in [H]$
, the seller sets a fixed price $D_{h} \in \mathcal{D}$, and the buyer decides on a binary sequence of  take-or-leave actions $\{z_{t}\}_{t\in [T]} \in \{0,1\}^{T}$.  Then
%  \widetilde{\mathcal{O}}\left(\frac{T^{1-\xi}}{|\mathcal{E}_{h}|} + T^{-\xi}\right)
we say a buyer's strategy is $\xi$-adaptive for $\xi \in (0,1)$ if
\begin{enumerate}
    \item \textbf{Adaptivity: } there exists a universal error function $\phi:\N \times \N \to [0,1]$ decreasing in the first argument such that for all episodes $h = 1, 2, \dots H$, $\left|\frac{1}{|\mathcal{E}_{h}|}\sum_{t\in \mathcal{E}_{h}}z_{t} - \frac{\rev(D_{h} )}{D_{h} }\right|\leq \phi(|\mathcal{E}_{h}|,T)$  w.p. at least $1-\frac{1}{T}$;\footnote{Note that $z_{t}$ for any $t\in \mathcal{E}_{h}$ would also depend on the price $D_{h}$.} 
    \item \textbf{Stability: } there exists a minimum episode length $E_{0}=\Omega(T^{1-\xi})$ such that $\phi(|\mathcal{E}_{h}|,T) < \frac{G}{2\Bar{d}}$  for any episode
$h$ whose length $|\mathcal{E}_{h}| \geq E_{0}$. Here $G \defeq \min_{d,\widetilde{d} \in \mathcal{D}:\rev(d) \neq \rev(\widetilde{d})}\left|\rev(d) - \rev(\widetilde{d})\right|$ is the minimum gap between any two non equal revenues corresponding to prices in $\mathcal{D}$. 
% \jason{Alternative for stability: there exists a minimum episode length $E_{0}=\Omega(T^{1-\xi})$ such that $\lim_{T\to \infty} \phi(|\mathcal{E}_{h}|,T) = 0$  for any episode
% $h$ whose length $|\mathcal{E}_{h}| \geq E_{0}$.}
\end{enumerate}
\end{definition}
Note that the  error function $\phi(|\mathcal{E}_{h}|,T)$ does not depend on the actual price $D_{h}$ set in episode $h \in [H]$.
The first adaptivity condition characterizes the buyer algorithm's ability to adapt and optimally react to prices across different episodes. The term $\left|\frac{D_{h}}{|\mathcal{E}_{h}|}\sum_{t\in \mathcal{E}_{h}}z_{t} - \rev(D_{h})\right|$ is the seller's average revenue loss, relative to the revenue from optimal buyers, over a certain period under fixed price $D_{h}$. However, the term can alternatively be viewed as the buyer's deviation from optimal behavior induced by the optimal threshold solution $\bm{x}_{D_{h}}$ because $\frac{\rev(D_{h})}{D_{h}} = \sum_{n \in [N]} \valpe^{n}x_{D_{h}}^{n}$ is the optimal probability of which the buyer should take price $D_{h}$. The first adaptivity condition hence states that the buyer's deviation from optimality under a fixed price is bounded. The second stability condition states that for long enough episodes, the deviation of buyer behavior from optimality stabilizes and reaches a certain low point, namely $\frac{G}{2\Bar{d}}$. Additionally, the stability condition states that a $\xi$-adaptive algorithm will require an order of $\Omega(T^{1-\xi})$ periods to stabilize. Thus, the larger $\xi$, the more stable the algorithm is.
Finally, we remark that if error function $\phi$  for some buyer algorithm is independent of $T$, then the stability condition would be easily satisfied. %For example,  if $\phi(|\mathcal{E}_{h}|,T) = \mathcal{O}({1}/{\sqrt{|\mathcal{E}_{h}|}})$, then the buyer's deviation from optimality would rapidly vanish, and eventually  $\phi(|\mathcal{E}_{h}|,T)$ would reach $\frac{G}{2\Bar{d}}$ in a constant amount of periods (i.e. for this algorithm $\xi = 1$). However, an error function typically depends on $T$  as they \negin{What is ``they"? buyer's algorithm?} adapt to episodic prices, as we will see in an example presented later.



%\jason{old version:
%Here, recall  the per-period revenue 
%$\rev(d) = d\sum_{n \in [N]} \valpe^{n}x_{d}^{n}$ where $\bm{x}_{d} \in \Delta_{N}$ is the unique optimal threshold vector solution to $\util(d)$, and hence  
%$\frac{\rev(d)}{d} = \sum_{n \in [N]} \valpe^{n}x_{d}^{n}$ is the optimal probability of which the buyer should take price $d$.  On the other hand, $\frac{1}{|\mathcal{E}_{h}| }\sum_{t\in \mathcal{E}_{h}}z_{t}$ \negin{You can call ``time-average of acceptance decisions $z_t$ during episode $\mathcal{E}_h$"} is the realized acceptance ratio, or proportion of periods in episode $\mathcal{E}_{h}$ that the buyer accepts price $D_{h}$. Therefore, the statement regarding $\left|\frac{1}{|\mathcal{E}_{h}| }\sum_{t\in \mathcal{E}_{h}}z_{t} - \frac{\rev(D_{h})}{D_{h}}\right|\leq \phi(|\mathcal{E}_{h}|,\delta)$ implies the realized acceptance ratio is close to the optimal acceptance probability for long enough episodes under the optimal threshold bidding strategy (see Lemma \ref{thm:optbidding}). \negin{Please discuss the second condition as well. You have sth below. But, make it clear this is the second condition.}
%We remark that the notion of adaptiveness pertains to an algorithm's ability to adopt to nonstationary environments. In particular, the parameter $\xi$ in the definition of adaptive strategies  can be interpreted as the order of periods (i.e. $T^{\xi}$) needed for the algorithm to stabilize and act near optimally after a change in the underlying occurrence distribution  $\bm{p} \in \Delta_{K}$ on $\mathcal{W}$.}


The main result of this subsection is presented in Theorem \ref{thm:episodicprice}, which characterizes the performance of our pricing algorithm against any $\xi$-adaptive buyer algorithm. The proof of Theorem \ref{thm:episodicprice} can be found in Appendix \ref{proof:thm:episodicprice}.
\begin{theorem}[Pricing against $\xi$-adaptive buyer strategies]
\label{thm:episodicprice}
Assume the buyer runs some $\xi$-adaptive
algorithm with error function $\phi$.
Fix $\epsilon \in (0,\xi)$ and let $T_{\epsilon} >0$ satisfy $\phi(T^{1-\xi + \epsilon},T) < \frac{G}{2\Bar{d}}$ for all $T >T_{\epsilon} $. \footnote{$T_{\epsilon}$ exists because the minimum episode length from the stability condition can be taken as $E_{0} = T^{1-\xi + \epsilon}$ for large enough $T$ so that $\phi(T^{1-\xi + \epsilon},T) < \frac{G}{2\Bar{d}}$. Here, we also used the fact that
$\phi$ is decreasing in its first argument. } 
Then, if the seller adopts the pricing strategy in Algorithm \ref{alg:pricing} with episode length $E = T^{1-\xi + \epsilon}$ over a time horizon $T >\max\left\{T_{\epsilon}, \left(4\Bar{d} \left\lfloor\log_{2}(M) \right\rfloor +4\Bar{d} \right)^{\frac{1}{\xi-\epsilon}}\right\}$, under Assumption \ref{assum:price:nontriv} the seller's regret is bounded as
\begin{align}
   \text{Reg}_{\text{sell}}\leq  2\Bar{d} \left(\left\lfloor\log_{2}(M) \right\rfloor + 1\right) \cdot T^{1-\xi + \epsilon}  + 2\Bar{d}T \cdot \phi\left(\frac{T}{2},T\right) + \Bar{d}\left(\left\lfloor\log_{2}(M)\right\rfloor + 1\right)^{2}/2\,.
\end{align}
\end{theorem}
{Theorem \ref{thm:episodicprice} delineates how a $\xi$-adaptive algorithm's adaptivity and stability properties factor into seller regret (see discussion after Definition \ref{def:robust} for details on adaptivity and stability). The first term $ T^{1-\xi + \epsilon}$ in the seller's regret corresponds to the buyer algorithm's stability property, which characterize its length of periods needed to stabilize in each episode;  the second term $\phi\left(\frac{T}{2},T\right) $  corresponds to the adaptivity property, which represents the buyer's deviation from the optimal threshold-based strategy characterized by the optimal solution $\bm{x}_{d}$ to $\util(d)$ for any price $d\in \mathcal{D}$. Finally, we remark that the seller does not need to know the exact value of $\xi$, as some lower bound $\xi$ would be sufficient.
}


% \negin{todo:Seller's regret = stabilization error + buyer's regret.} Theorem \ref{thm:episodicprice} delineates the  connection between the regret of our proposed pricing algorithm and the buyer's regret in a stationary fixed price environment.
% In particular, assume the price is fixed at $d$ \negin{Please use $d$ as before} throughout $T$ periods, then 
% \begin{align}
%     \left|T\cdot \util(D) -\sum_{t\in [T]}v_{t} z_{t}\right|=\left|T\sum_{n \in [N]} \valpe^{n}\V^{n}x_{D}^{n} - \sum_{t\in [T]}v_{t} z_{t}\right| \leq \Bar{v} T\left|\frac{\rev(D)}{D} - \frac{1}{|T|}\sum_{t\in [T]}z_{t} \right|\leq \Bar{v}T\phi(T,\delta)\,,
% \end{align}
% where $\Bar{v}$ is the maximum possible valuation.
% Therefore, the term $T\phi(T,\delta)$ in the seller's regret exactly corresponds to the buyer's regret assuming the buyer faces a fixed price over the entire horizon. 


We note that $\xi$-adaptivity is not at all restrictive. %To provide an example by relating to our proposed $\textsc{CTBR}_{\algo}$ framework in Section \ref{sec:algo}, and to put Theorem \ref{thm:episodicprice} in context, we show that in an ``episodic'' non-stationary environment,
We will show that our $\textsc{CTBR}_{\algo}$ coupled with the simple SGD learning algorithm and constant step sizes is $\frac{1}{3}$-adaptive. 

% \begin{theorem}[Near-optimal regret in non-stationary stochastic environment]
% \label{thm:constraintrobustnonstat}
% Fix a sequence of distributions $\bm{p}_{t} \in \Delta_{K} $ and consider $(v_{t},d_{t})$ being drawn independently from $\bm{p}_{t}$ for each $t \in [T]$. Define $\overline{\bm{p}} = \frac{1}{T}\sum_{t\in [T]} \bm{p}_{t}$ and
% $S = \sum_{t\in [T]} \norm{\bm{p}_{t} -\overline{\bm{p}}}_{1}$. Then the regret of $\textsc{CTBR}_{\algo^{\OMD}}$ is given by
% \begin{align}
%     \E\left[P(\left\{v_{t},d_{t}\right\}_{t\in [T]};\alpha,\gamma,\rho)  - \sum_{t\in[T]} \left(v_{t} - \alpha d_{t}\right)\I\left\{b_{t} \geq d_{t}\right\} \right] \leq S\max_{k\in [K]}\left\{v^{k} - \alpha d^{k}\right\} + \mathcal{O}\left(T\ell^{\algo^{\text{OMD}}}\left(T,\delta\right)\right)\,,
% \end{align}
% w.p. at least $1-\delta$.
% \end{theorem}

\begin{theorem}[$\textsc{CTBR}$ with constant step size SGD is $\frac{1}{3}$-adaptive]
\label{thm:CTBRadapt}
There exists some $T_{0} \in \N$ such that for all $T > T_{0}$, $\textsc{CTBR}$ equipped with SGD with constant step size $\eta = T^{-\frac{2}{3}}$ is $\frac{1}{3}$-adaptive. The corresponding minimum episode length can be taken as $E_{0} = T^{\frac{2}{3} + \epsilon}$ for some $\epsilon = \Theta(1/\log(T))$ and $\epsilon < 1/3$.
% Now assuming the buyer runs $\textsc{CTBR}$ with SGD and constant step size  $\eta = T^{-\frac{2}{3}}$, and the seller sets prices with episode length $E = T^{\frac{2}{3}+\epsilon}$  for some fixed $\epsilon \in (0,\frac{1}{3})$ using Algorithm \ref{alg:pricing}, then there exists some $T_{\epsilon}>\left(4\Bar{d} \left\lfloor\log_{2}(M) \right\rfloor +4\Bar{d} \right)^{\frac{1}{\frac{1}{3}-\epsilon}}  $ such that for all $T > t_{\epsilon}$ the seller's regret is bounded as
% \begin{align}
%   \text{Reg}_{\text{sell}}\leq  2\Bar{d} \left(\left\lfloor\log_{2}(M) \right\rfloor + 1\right) \cdot T^{\frac{2}{3} + \epsilon}  + 4\Bar{d}\sqrt{T\log\left(2T^{2}\right)} +  \frac{\mathcal{T}}{2} +C\left(A +B\right)T^{\frac{2}{3}} + \Bar{d}\left(\left\lfloor\log_{2}(M)\right\rfloor + 1\right) ^{2} = \Theta(T^{\frac{2}{3}+\epsilon})\,,
% \end{align}
% where $A,B,C,\marg$ are the same as those in Theorem \ref{thm:OMDregret}, and $\mathcal{T} = \min\left\{t \in [T]: A\left(1-2T^{-\frac{2}{3}}\right)^{t} + BT^{-\frac{1}{3}}<S \right\} =\Theta(T^{\frac{1}{3}})$.
\end{theorem}

% \begin{theorem}[$\textsc{CTBR}_{\algo}$ with constant step size SGD is $\frac{1}{3}$-adaptive]
% \label{thm:constraintrobustnonstat}\negin{Can you just say CTBR with this step size is $1/3$ robust and assuming buyer runs this algorithm, the seller's regret is this.}
% Let $A,B,C,\marg$ be defined as in Theorems \ref{thm:biddingRegret} and \ref{thm:OMDregret}, and $\mathcal{T} = \min\left\{t \in [T]: A\left(1-2T^{-\frac{2}{3}}\right)^{t} + BT^{-\frac{1}{3}}<S \right\} =\Theta(T^{\frac{1}{3}})$.  Define 
% \begin{align}
%     \phi(\tau,T) = \sqrt{\frac{2\log\left(2T^{2}\right)}{\tau}} + \frac{\mathcal{T}}{\tau } +C\left(\frac{AT^{\frac{2}{3}}}{2\tau} +BT ^{-\frac{1}{3}}\right) = \Theta\left(\frac{1}{\sqrt{\tau}} + \frac{T^{\frac{2}{3}}}{\tau}+ T ^{-\frac{1}{3}}\right)\,,
% \end{align}
% and for any fixed $\epsilon \in (0,\frac{1}{3})$, assume that entire time horizon $T$ is large such that $\phi(T^{\frac{2}{3}+\epsilon},T) = \Theta(T ^{-\epsilon})<  \frac{G}{2\Bar{d}}$. If the entire $T$ periods is divided into $S$ consecutive episodes $\mathcal{E}_{1} \dots \mathcal{E}_{H}$, and the buyer runs $\textsc{CTBR}_{\algo}$ with SGD and constant step  size $\eta = T^{-\frac{2}{3}}$, then
% \begin{enumerate}
%     \item [(1)] $\left|\frac{1}{|\mathcal{E}_{h}|}\sum_{t\in \mathcal{E}_{h}}z_{t} - \frac{\rev(D_{h})}{D_{h}}\right|\leq \phi(|\mathcal{E}_{h}|,T)$ for any episode $h \in [H]$ w.p. at least $1-\frac{1}{T}$;
%     \item [(2)]$\phi(|\mathcal{E}_{h}|,T)< \frac{G}{2\Bar{d}}$ for any episode
% $h$ whose length $|\mathcal{E}_{h}| \geq T^{\frac{2}{3}+\epsilon}$
% \end{enumerate}
% This implies that $\textsc{CTBR}_{\algo}$ with SGD and constant step size is $\frac{1}{3}$-adaptive.
% \end{theorem}

The proof for Theorem \ref{thm:CTBRadapt} is provided in Appendix \ref{proof:thm:CTBRadapt}.
We remark that although SGD with constant step size is adaptive, SGD with vanishing step size is not adaptive. To see this intuitively, consider the entire horizon $T$ being split equally into two halves. Suppose that  the difference between the prices in the two halves is large. From Theorem \ref{thm:OMDregret}, we know that SGD with vanishing step size adjusts to the fixed price quickly at a $\frac{1}{\sqrt{t}}$ rate in the first half. But when the algorithm enters the second half, all step sizes are less than $\frac{2}{T}$, which does not provide enough flexibility for the algorithm to adapt to the new price.


\begin{corollary}[Seller's regret against $\textsc{CTBR}_{\algo}$ with constant step size SGD]
\label{corr:constantSGDsellerRegret}
Let $T > T_{0}$ where $T_{0}$ is defined in Theorem \ref{thm:CTBRadapt}. Assume the buyer runs $\textsc{CTBR}_{\algo}$ with SGD and constant step  size $\eta = T^{-\frac{2}{3}}$. Then for a fixed $\epsilon \in (0,\frac{1}{3})$ and $\epsilon = \Theta(1/\log(T))$, if  the seller sets prices with episode length $E = T^{\frac{2}{3}+\epsilon}$
using Algorithm \ref{alg:pricing}, then for all $T> \max\left\{T_{0},\left(4\Bar{d} \left\lfloor\log_{2}(M) \right\rfloor +4\Bar{d} \right)^{\frac{1}{\frac{1}{3}-\epsilon}}\right\}$, the seller's regret is bounded as
\begin{align*}
  \text{Reg}_{\text{sell}}\leq  2\Bar{d} \widetilde{H} \cdot T^{\frac{2}{3} + \epsilon}  + 4\Bar{d}\sqrt{T\log\left(2T^{2}\right)} +  \frac{\mathcal{T}}{2} +C\left(\widetilde{A} +\widetilde{B}\right)T^{\frac{2}{3}} + \Bar{d}\widetilde{H}^{2}/2 = \Theta(T^{\frac{2}{3}+\epsilon})\,,
\end{align*}
where $\widetilde{H} = \left\lfloor\log_{2}(M) \right\rfloor + 1$, $C$ and $\marg$ are defined as in Theorem \ref{thm:OMDregret}, $\widetilde{A}= \sqrt{2+ 16\sqrt{\log\left(T^{2}\log\left(T\right)\right)}}$, 
$\widetilde{B} = 2\sqrt{\left(1+72\log\left(T^{2}\log\left(T\right)\right)\right)}$, 
% \begin{align}
%     \widetilde{A}= \sqrt{2+ 16\sqrt{\log\left(T^{2}\log\left(T\right)\right)}},\quad \widetilde{B} = 2\sqrt{\left(1+72\log\left(T^{2}\log\left(T\right)\right)\right)}\,,
% \end{align}
and $\mathcal{T} = \min\left\{t \in [T]: \widetilde{A}\left(1-2T^{-\frac{2}{3}}\right)^{t} + \widetilde{B}T^{-\frac{1}{3}}<S \right\} =\Theta(T^{\frac{1}{3}})$.
% Fix $\epsilon \in (0,\frac{1}{3})$ and assume the horizon $T$ is large such that $\phi(T^{\frac{2}{3}+\epsilon},T) <\frac{G}{2\Bar{d}} $ where $\phi$ is defined in  Theorem \ref{thm:constraintrobustnonstat}, and $T > \left(4\Bar{d} \left\lfloor\log_{2}(M) \right\rfloor +4\Bar{d} \right)^{\frac{1}{\frac{1}{3}-\epsilon}} $. If and the seller sets prices with episode length $E = T^{\frac{2}{3}+\epsilon}$
% using Algorithm \ref{alg:pricing}, then the seller's regret is bounded as
% \begin{align}
%   \text{Reg}_{\text{sell}}\leq  2\Bar{d} \left(\left\lfloor\log_{2}(M) \right\rfloor + 1\right) \cdot T^{\frac{2}{3} + \epsilon}  + 4\Bar{d}\sqrt{T\log\left(2T^{2}\right)} +  \frac{\mathcal{T}}{2} +C\left(A +B\right)T^{\frac{2}{3}} + \Bar{d}\left(\left\lfloor\log_{2}(M)\right\rfloor + 1\right) ^{2} = \Theta(T^{\frac{2}{3}+\epsilon})\,,
% \end{align}
% where $A,B,C,\mathcal{T}$ are the same as those in Theorem \ref{thm:OMDregret}.
\end{corollary}

The proof for Corollary \ref{corr:constantSGDsellerRegret} can be found in Appendix \ref{corr:proof:constantSGDsellerRegret}.






==> Scratch1_4_impossible.tex <==
Having presented a fairness guarantee in the previous Section \ref{sec:VCG} that improves according to the platform's ML advice accuracy, a natural question is that for a given level of accuracy $\beta$, \jason{can one achieve a universally better fairness guarantee than that of} Theorem \ref{thm:fairnessbound} via considering auction formats other than VCG? In this section, we demonstrate that the answer is negative when we restrict the auction to a broad class of mechanisms that are anonymous, truthful and possibly randomized. \jason{Here, we again emphasize that truthfulness is w.r.t. quasi-linear utility maximizers.} To show this result, our strategy is to construct an autobidding instance with any auction format that belongs to  the aforementioned class of mechanisms, and argue that there is at least a bidder $i$ who will incur a welfare loss at least $\frac{1-\beta}{\alpha_{i}-1}\opt_{-i}$, which is the welfare loss upper bound shown in Theorem \ref{thm:fairnessbound}. 

The class of anonymous, truthful and randomized
mechanisms is extremely large, and therefore
to construct a suitable autobidding instance, we will rely on several simple yet fundamental definitions and properties for such class of auctions. Note that these properties are standard; see e.g. \cite{mehta2022auction}.
\begin{definition}[Anonymous auction]
Consider any auction mechanism $\mathcal{M}$ whose (possibly random) allocation $\mathcal{X}:\R^{N}\to \R^{N}$ satisfies $\sum_{i\in[N]}\mathcal{X}_{i}(\bm{b}) = 1$ for any number of bidders $N$ and bid profile $\bm{b} \in \R_{\geq 0}^{N}/\{\bm{0}\}$. Then we say $\mathcal{M}$ is anonymous if the outcome for a permutation of any bid profile $\bm{b}$ is the permutation of the outcome for $\bm{b}$, i.e. for any permutation $\sigma: [N]\to [N]$, then $\left[\mathcal{X}(b_{\sigma(1), \dots \sigma(N)})\right]_{i} = \left[\mathcal{X}(\bm{b})\right]_{\sigma(i)} $ for any $i \in [N]$.
\end{definition}
As an example, a single second price auction with an identical reserve price (which can still be
$\beta$-approximate for all bidders \yuan{This would in general violate the upper bound in the definition of $\beta$-approximation for some bidders? Maybe highlight that this property holds in the example you constructed below.}) is anonymous.

The following lemma shows that for anonymous and truthful auctions, the probability of the lowest bidder winning a single auction is capped by a bound that decreases as the number of bidders grow.
\begin{lemma}
\label{lem:winprobub}
In an anonymous and truthful auction for a single item with $N$ bidders, the bidder who submits the lowest bid wins the item with probability at most $\frac{1}{N}$.
\end{lemma}

The final technical definition and lemma (i.e. Definition \ref{def:monop} and Lemma \ref{lem:singlebiddercost}) concerns the scenario where only one bidder participates in the auction (others bid 0), and present an upper bound on the probability and cost  respectively for the single bidder to win the auction.
\begin{definition}[Single bidder purchase probability and bid threshold]
\label{def:monop}
For any anonymous and truthful auction $\mathcal{M}$, consider the setting with a single bidder. Let $b > 0$ be the submitted bid, and define 
\begin{align}
    \pi_{\mathcal{M}} = \lim_{b\to \infty}\prob(\text{bidder wins item with bid $b$})\,,
\end{align}
where the limit exists because in a truthful auction, $\prob(\text{bidder wins item with bid $b$})$ increases in $b$. Assume this max probability is reached at some bid threshold $Q_{\mathcal{M}}$, i.e.
\begin{align}
   Q_{\mathcal{M}} = \min\left\{b>0: \prob(\text{bidder wins item with bid $b$}) =  \pi_{\mathcal{M}}\right\} \,.
\end{align}
\end{definition}
Note that in a deterministic single-slot auction that allocates to the highest bidder,  $\pi_{\mathcal{M}} = 1$, and $Q_{\mathcal{M}}  \to 0$. For example, in an SPA, the single bidder can win the auction with any arbitrarily small positive bid with probability 1.
\begin{lemma}[Lemma 4 in \cite{mehta2022auction}]
\label{lem:singlebiddercost}
For any anonymous and truthful auction $\mathcal{M}$ with single-bidder purchase probability $ \pi_{\mathcal{M}}$ and bid threshold $ Q_{\mathcal{M}}$, the expected cost for a single bidder for winning the item is at most $\pi_{\mathcal{M}} \cdot Q_{\mathcal{M}}$.
\end{lemma}


Our main result for this section is the following Theorem \ref{thm:imposs}, where we present an autobidding instance w.r.t. to any anonymous, truthful, and possibly randomized auction in which there must exist a bidder $i$ who will incur a welfare loss at least $\frac{1-\beta}{\alpha_{i}-1}\opt_{-i}$, which is the welfare loss upper bound in Theorem \ref{thm:fairnessbound}. 
\begin{theorem}
\label{thm:imposs}
For any auction $\mathcal{M}$ that is anonymous, truthful, and possibly randomized, consider an autobidding problem instance w.r.t.  $\mathcal{M}$ with $M = 2K+1$ auctions and $N = K+1$ bidders. Fix bidder 0's bid multiplier to be $\alpha_{0}$ and some $\beta\in [0,1)$. Consider the bidder values $\{v_{i,j}\}_{i\in[N],j\in[M]}$, and assume in each auction $j$ we impost a single reserve $r_{j}$, both given in the following table.
\renewcommand{\arraystretch}{2}
\begin{center}
\begin{tabular}{|c | c c c c c c c c c|} 
 \hline
  & $A_{1}$ & $A_{2}$ & \dots  &   $A_{K}$  & $A_{K+1}$ & $A_{K+2}$ & \dots & $A_{2K}$ &  $A_{2K+1}$\\
 \hline\hline
 $B_{0}$ & $v$ & $v$ & \dots & $v$ & 0 & 0 & \dots & 0  & $X$\\ 
 \hline
$B_{1}$  & $\frac{\alpha_{0}v+\epsilon}{\rho}$ & $\frac{\alpha_{0}v+2\epsilon}{\rho}$  & \dots &  $\frac{\alpha_{0}v+K\epsilon}{\rho}$ & $\gamma$  & 0 &  \dots & 0 & 0\\
  \hline
 $B_{2}$  & $\frac{\alpha_{0}v+2\epsilon}{\rho}$ & $\frac{\alpha_{0}v+3\epsilon}{\rho}$  & \dots &  $\frac{\alpha_{0}v+\epsilon}{\rho}$ & 0 &  $\gamma$ & \dots &  0 & 0  \\
 \hline
 \vdots & \vdots &  \vdots  &  &   \vdots  &  \vdots & \vdots & & \vdots & \vdots \\
  \hline
   $B_{K}$  & $\frac{\alpha_{0}v+K\epsilon}{\rho}$ & $\frac{\alpha_{0}v+\epsilon}{\rho}$  & \dots &  $\frac{\alpha_{0}v+(K-1)\epsilon}{\rho}$ & 0  & 0  & \dots & $\gamma$ & 0\\
   \hline
   \hline
   Reserve & $\beta v$ & $\beta v$  & \dots & $\beta v$  & $\beta \gamma$ &  $\beta \gamma$ & \dots &  $\beta \gamma$ & $\beta X$\\
   \hline
\end{tabular}
\end{center}
In the table, we let $\gamma > \frac{Q_{\mathcal{M}}}{\beta} > Q_{\mathcal{M}}$, $\epsilon = O(1/K^{3})$ and $v = \frac{1-\beta}{\alpha_{0}-1}\cdot \pi_{\mathcal{M}}\cdot \gamma$. Let $\rho,X$ and a large enough $K$ satisfy the following:
\begin{align}
\begin{aligned}
\label{eq:imposs:params}
%   & \gamma \geq \max\left\{\frac{1}{(1-\beta)\pi_{\mathcal{M}}}\left( \frac{(1-\beta)\alpha_{0}}{\alpha_{0}-1} + \frac{(K+1)K}{2}\epsilon\right),\frac{Q_{\mathcal{M}}}{\beta} \right\}\\ 
   & \alpha_{0}<\rho <\frac{\alpha_{0}}{\beta} ~\text{s.t.}~\frac{\alpha_{0}v+K\epsilon}{\rho} < v,\quad \text{ and } X > \max\left\{\frac{Q_{\mathcal{M}}}{\alpha_{0}}, \frac{\alpha_{0}v}{\pi_{\mathcal{M}}}\right\}\,.
  \end{aligned}
\end{align}
 Then, letting the (possibly random) outcome be $\bm{x}$ when bidders 1, ... K all adopt the bid multiplier $\rho$, 
 the ROI constraints for all bidders are satisfied when $K\to\infty$ and $\rho \to \alpha_{0}$, and for bidder $0$ we have 
 \begin{align}
    \lim_{K\to \infty} \frac{\E_{\mathcal{M}}[\loss_{0}(\bm{x})]}{\E_{\mathcal{M}}\left[\opt_{-0}\right]} \geq \frac{1-\beta}{\alpha_{0}-1}\,,
 \end{align}
 where $\E_{\mathcal{M}}$ is taken w.r.t the randomness in outcome $\bm{x}$ due to randomness in the auction $\mathcal{M}$, and the loss of bidder 0, namely $\loss_{0}$, is defined in Equations (\ref{eq:loss}).
%  fairness guarantee is at most $1-\frac{1-\beta}{\alpha_{0}-1}\cdot \frac{\opt_{-0}}{\opt_{0}}$.
\end{theorem}
\begin{remark}
Note that  in each auction $j\in[M]$, we impose a single reserve price $r_{j}$, which maintains the anonymity for each auction. Further,  price $ r_{j} \in [\beta v_{i,j}, v_{i,j})$ for any $i \in [N]$ and $v_{i,j}\neq 0$, so these reserve prices are $\beta$-approximate (see Definition \ref{def:reserve}). 
\end{remark}

The proof of Theorem \ref{thm:imposs} is presented in Appendix \ref{pf:thm:imposs}. Since
VCG is also truthful and anonymous, 
Theorem \ref{thm:imposs} along with Theorem \ref{thm:fairnessbound} implies that with $\beta$-accurate ML advice, VCG achieves the best possible fairness guarantee among the broad class of anonymous, truthful and possibly randomized auctions.



==> Scratch1_imposs.tex <==
\subsection{Proof of Theorem \ref{thm:imposs}}
\label{pf:thm:imposs}

\begin{proof}
First note that bidder 0 only has competition in auctions $A_{1}...A_{K}$, and hence can only incur a loss (that contributes to $\loss_{0}(\bm{x})$ defined in  Equations (\ref{eq:loss})) within these auctions. Hence $ \E_{\mathcal{M}}[\loss_{0}(\bm{x})]  =  v\sum_{j\in [K]}\prob(\text{bidder 0 loses auction $j$})$. Then we consider the following:
\begin{align}
\begin{aligned}
    \E_{\mathcal{M}}[\loss_{0}(\bm{x})] ~=~ &  v\sum_{j\in [K]}\prob(\text{bidder 0 loses auction $j$})~=~  v\sum_{j\in [K]}\left(1-\prob(\text{bidder 0 wins auction $j$})\right)\\
    ~\overset{(a)}{\geq}~ & v \cdot \frac{K^{2}}{K +1} = \frac{1-\beta}{\alpha_{0}-1}\cdot \gamma \cdot \pi_{\mathcal{M}} \cdot \frac{K^{2}}{K +1} =  \frac{1-\beta}{\alpha_{0}-1} \cdot \E_{\mathcal{M}}\left[\opt_{-0}\right] \cdot \frac{K}{K+1}\,.
    % > \frac{1-\beta}{\alpha_{0}-1}\gamma (K-1) = \frac{1-\beta}{\alpha_{0}-1}\opt_{-0}
    \end{aligned}
\end{align}
Here (a) holds because bidder 0 bids $\alpha_{0}v$ for any auction in 1,2...K, which is strictly less than all other bidders' bids as they all adopt  multipliers $\rho$ in these auctions, so from Lemma \ref{lem:winprobub}, we have $\prob(\text{bidder 0 wins auction $j$})\leq \frac{1}{K+1}$.

Therefore we have 
\begin{align}
    \lim_{K\to \infty}\frac{\E_{\mathcal{M}}[\loss_{0}(\bm{x})]}{\E_{\mathcal{M}}\left[\opt_{-0}\right]} \geq \frac{1-\beta}{\alpha_{0}-1}\cdot  \frac{K}{K+1} =  \frac{1-\beta}{\alpha_{0}-1}\,.
\end{align}

Now it only remains to show that the multiplies $(\alpha_{0}, \rho, \dots \rho) \in (1,\infty)^{K+1}$ yields a feasible outcome, i.e. the ROI constraints of each bidder is satisfied in expectation. Let $V_{i,j}$ and $C_{i,j}$  be the expected value and cost of bidder $i$ in auction $A_{j}$, respectively.

\textbf{1. Showing bidder $0$'s ROI constraint is satisfied}.
We show by the following: bidder 0 only incurs a non-zero expected cost in auctions $A_{1}\dots A_{K}$ and $A_{2K+1}$, and we will show that the expected value $V_{0,2K+1}$ is lower bounded by the expected costs $C_{0,2K+1} + \sum_{j\in[K]}C_{0,j}$.

Since $\alpha_{0}X  > Q_{\mathcal{M}}$, the definition of the single-bidder purchasing probability in Definition \ref{def:monop} implies that  bidder 0 acquires an expected value from  auction $A_{2K+1}$ of $V_{0,2K+1} = \pi_{\mathcal{M}}X$. Further,  since bidder 0 is submits the lowest bids in auctions $A_{1} \dots A_{K}$ under bid multiplier profile $(\alpha_{0},\rho \dots \rho)\in (0,\infty)^{K+1}$,  from Lemma \ref{lem:winprobub}, we have $\prob(\text{bidder 0 wins auction $j$})\leq \frac{1}{K+1}$ for all $j \in [K]$. Since the payment of a bidder in an auction is at most her submitted bid, we know that $\sum_{j \in [K]}C_{0,j}\leq  K\cdot \frac{\alpha_{0}v}{K+1} < \pi_{\mathcal{M}}X = V_{0,2K+1}$, where the inequality follows from the definition of $X$ in Equation (\ref{eq:imposs:params}) such that $X > \max\left\{\frac{Q_{\mathcal{M}}}{\alpha_{0}}, \frac{\alpha_{0}v}{\pi_{\mathcal{M}}}\right\}$. This implies bidder 0's ROI constraint is satisfied.

\textbf{2. Showing bidder $i$'s ROI constraint is satisfied for any $i = 1,2 \dots K$}. We show by considering the following: bidder $i$ only incurs a non-zero expected cost in auctions $A_{1}\dots A_{K}$ and $A_{K+i}$, and we will show that the expected values $ \sum_{k\in [K+1]}V_{i,j}$ is lower bounded by the expected costs $C_{i,K+i} + \sum_{j\in[K]}C_{i,j}$.

\begin{itemize}
 
    \item \textbf{Calculate cost $C_{i,K+i}$: } For auction $A_{K+i}$, bidder $i$'s bid is $\rho\gamma > \gamma > Q_{\mathcal{M}}$ from the definition of $\gamma$, so by Definition \ref{def:monop}, the probability of $i$ winning the item in auction $A_{K+i}$ is $\pi_{\mathcal{M}}$, and the expected cost is
    \begin{align}
    \label{eq:imposs:costub}
     C_{i,K+i} \leq \pi_{\mathcal{M}}\cdot \max\left\{r, Q_{\mathcal{M}}  \right\} \leq \pi_{\mathcal{M}}\cdot\beta \gamma\,,
     \end{align}
     where the final inequality follows from the definition $r = \beta\cdot \min_{i\in[N],j\in[M]}v_{i,j}  $
     
     \item \textbf{Upper bound costs $\sum_{j\in[K]}C_{i,j}$: }  
             For auctions $[K] = 1\dots K$,  bidder $i$'s total expected cost can be bounded as
        \begin{align}
        \begin{aligned}
        \label{eq:imposs:costub2}
           \sum_{j\in[K]} C_{i,j} ~\leq~ & \rho \sum_{j\in[K]} v_{i,j} \prob\left(\text{bidder $i$ wins auction $A_{j}$}\right)\\
           ~\leq~ & \alpha_{0}v \sum_{j \in [K]}\prob\left(\text{bidder $i$ wins auction  $A_{j}$}\right) + \frac{(K+1)K}{2}\epsilon \\
            ~\overset{(a)}{\leq}~ & \alpha_{0}v+ \frac{(K+1)K}{2}\epsilon \\
           \end{aligned}
        \end{align}
        In (a) we used the fact that $ \sum_{j \in [K]}\prob\left(\text{bidder $i$ wins auction  $A_{j}$}\right)\leq 1 $ due to the following:
        
        Consider the bid profile $\bm{b} = (\alpha_{0}v, \alpha_{0}v+\epsilon, \alpha_{0}v+2\epsilon \dots \alpha_{0}v+ K\epsilon)\in \R_{+}^{K+1}$. By anonymity of auction $\mathcal{M}$, there exists probabilities $\bm{q}(\bm{b})=(q_{0}(\bm{b}),q_{1}(\bm{b}) \dots q_{K}(\bm{b})) \in [0,1]^{K+1}$ where $$q_{k}(\bm{b}) = \prob(\text{bid value $b_{k}$ wins auction $\mathcal{M}$ given competing bids $\bm{b}_{-k}$}) \quad \text{ and } \sum_{k=0}^{K}q_{k}(\bm{b})= 1.$$
        By recognizing $\bm{b}$ is exactly the set of bids in each auction $A_{1} \dots A_{K}$ under bid multipliers $(\alpha_{0},\rho,\dots \rho)\in (1,\infty)^{K+1}$, we know that
        \begin{align}
        \label{eq:imposs:competewinbound}
            \sum_{j \in [K]}\prob\left(\text{bidder $i$ wins auction $j$}\right) =  \sum_{k = 1}^{K} q_{k}(\bm{b}) = 1-  q_{0}(\bm{b})\leq 1
        \end{align}
       
     \item \textbf{Calculate $V_{i,K+i}$: }
        Considering auction $A_{K+i}$, bidder $i$ is the only bidder, and since $\rho \gamma >\gamma > Q_{\mathcal{M}}$, the definition of the single-bidder purchasing probability in Definition \ref{def:monop} implies that  bidder $i$'s acquires an expected value from this auction of 
    \begin{align}
    \label{eq:imposs:vallb}
        V_{i,K+i} = \pi_{\mathcal{M}}\cdot \gamma\,.
    \end{align} 
    
    \item \textbf{Lower bound $\sum_{k\in [K]}V_{i,j}$: }
    
    \begin{align}
    \label{eq:imposs:vallb2}
        \sum_{k\in [K]}V_{i,j} \geq \frac{\alpha_{0}v}{\rho}\sum_{j\in [K]}\prob\left(\text{bidder $i$ wins auction $j$}\right) \overset{(a)}{=} \frac{\alpha_{0}v}{\rho} \left(1-q_{0}(\bm{b})\right) \overset{(b)}{\geq} \frac{\alpha_{0}v}{\rho} \cdot \frac{K}{K+1}
    \end{align}
    where (a) follows from Equation (\ref{eq:imposs:competewinbound}) where we
    upper bounded $\sum_{j\in[K]}C_{i,j}$ and recall $\bm{b}= (\alpha_{0}v, \alpha_{0}v+\epsilon, \alpha_{0}v+2\epsilon \dots \alpha_{0}v+ K\epsilon)\in \R_{+}^{K+1}$; (b)
    follows from Lemma \ref{lem:winprobub} s.t. $q_{0}(\bm{b})\leq \frac{1}{K+1}$. This is 
    because $q_{0}(\bm{b})$ is the probability of winning with bid value $\alpha_{0}v$ when the other bids $(\alpha_{0}v+\epsilon, \alpha_{0}v+2\epsilon \dots \alpha_{0}v+ K\epsilon)\in \R_{+}^{K}$ are all greater than $\alpha_{0}v$.
\end{itemize}

Combining Equations  (\ref{eq:imposs:costub}),(\ref{eq:imposs:costub2}),(\ref{eq:imposs:vallb}) and (\ref{eq:imposs:vallb2}), we get
\begin{align*}
     & \sum_{j\in[K]}V_{i,j}  + V_{i,K+i} -  \left(\sum_{j\in[K]}C_{i,j}+ C_{i,K+i}\right) \\   
     ~\geq~ & \pi_{\mathcal{M}}\cdot \gamma  +\frac{\alpha_{0}v}{\rho} \cdot \frac{K}{K+1} - \left(\pi_{\mathcal{M}}\cdot\beta \gamma + \alpha_{0}v +  \frac{(K+1)K}{2}\epsilon\right)\\
     ~=~ &  \pi_{\mathcal{M}}\cdot (1-\beta) \gamma - \left(\alpha_{0}- \frac{\alpha_{0}}{\rho}\cdot \frac{K}{K+1} \right) v -  \frac{(K+1)K}{2}\epsilon\\
     ~=~ &  (\alpha_{0}-1)v - \left(\alpha_{0}- \frac{\alpha_{0}}{\rho}\cdot \frac{K}{K+1} \right) v -  \frac{(K+1)K}{2}\epsilon\,,
\end{align*}
where the final equality follows from the definition $v = \frac{1-\beta}{\alpha_{0}-1}\cdot \pi_{\mathcal{M}}\cdot \gamma$.

Finally, by taking $\rho \to \alpha_{0}$ and $K\to\infty$, and utilizing $\epsilon = O(1/K^{3})$ we have
\begin{align*}
& \lim_{\rho \to \alpha_{0}} \lim_{K\to\infty}\sum_{j\in[K]}V_{i,j}  + V_{i,K+i} -  \left(\sum_{j\in[K]}C_{i,j} C_{i,K+i}\right)~\geq~ 0 \,.
\end{align*}
This shows that bidder $i$'s ROI constraint is satisfied.

\end{proof}

==> Scratch1_model.tex <==
Consider $N$ bidders bidding in a single second price auction (SPA) without reserve. Let $\budget_{i} \in (0,1)$ be the budget rate and $\gamma_{i} \in (1,\infty)$ be the target ROI  for bidder $i\in [N]$. Assume all bidders adopt a uniform bidding strategy with bid multiplier $\alpha_{i} \in \mathcal{A} \defeq \{\alpha^{1}\dots \alpha^{K}\}$. The value of bidder $i$, namely $v_{i}$ is sampled independently from support $\mathcal{V}\subseteq [0,1]$ according to some distribution $P$ (common to all bidders).

The expected value $F_{i}(\mu_{i},\bm{\mu}_{-i})$, and  the expected realized expenditure $G_{i}(\mu_{i},\bm{\mu}_{-i})$ under the decision profile $\bm{\mu} \in \mathcal{A}^{N}$ as followed:
\begin{align}
    &F_{i}(\mu_{i},\bm{\mu}_{-i}) = \E\left[v_{i} \cdot \I\{\alpha_{i}v_{i}\geq \max_{j\neq i}  \alpha_{j}v_{j}\}\right]\\
    &G_{i}(\mu_{i},\bm{\mu}_{-i})= \E\left[\max_{j\neq i} \alpha_{j}v_{j} \cdot \I\{ \alpha_{i}v_{i} \geq \max_{j\neq i} \alpha_{j}v_{j}\}\right]
\end{align}
Here, the expectation is taken w.r.t. the randomness in $\bm{v}\in \mathcal{V}^{N}$.

Given the budget and ROI constraints of a bidder $i\in[N]$, under the multiplier decisions $\bm{\mu}_{-i}$ of other bidders, the feasible set of multipliers for $i$ is 
\begin{align}
   & \feasible_{i}(\bm{\mu}_{-i}) = \left\{\mu_{i} \geq 0: F_{i}(\mu_{i},\bm{\mu}_{-i})  -\gamma_{i}\cdot G_{i}(\mu_{i},\bm{\mu}_{-i})\geq 0 \text{ and }  G_{i}(\mu_{i},\bm{\mu}_{-i})\leq \budget_{i} \right\}\\
    & \feasible = \left\{\bm{\mu} \geq 0: \mu_{i} \in  \feasible_{i}(\bm{\mu}_{-i})\quad  \forall i\in [N]\right\}\,.
\end{align}
Therefore, bidder $i$'s optimization problem can be written as
% \begin{align}
%     \max_{\mu_{i}\in  \feasible_{i}(\bm{\mu}_{-i})}U_{i}(\bm{\mu}) ~=~& \max \quad \E\left[(v_{i} - \max_{j\neq i}  \alpha_{j}v_{j})\cdot \I\{ \alpha_{i}v_{i}\geq \max_{j\neq i}  \alpha_{j}v_{j}\}\right]\\
%     \text{s.t. } & \quad  \E\left[(v_{i} - \gamma_{i} \cdot \max_{j\neq i}  \alpha_{j}v_{j})\cdot \I\{ \alpha_{i}v_{i} \geq \max_{j\neq i}  \alpha_{j}v_{j}\}\right]\geq 0\\
%     & \quad  \E\left[ \max_{j\neq i}  \alpha_{j}v_{j}\cdot \I\{ \alpha_{i}v_{i}\geq \max_{j\neq i}  \alpha_{j}v_{j}\}\right]\leq \budget_{i}
% \end{align}
% By denotin we can rewrite
\begin{align}
    \max_{\mu_{i}\in  \feasible_{i}(\bm{\mu}_{-i})}F_{i}(\mu_{i},\bm{\mu}_{-i}) 
    ~=~ \max & \quad F_{i}(\mu_{i},\bm{\mu}_{-i})\\
    \text{s.t. } & \quad  F_{i}(\mu_{i},\bm{\mu}_{-i})  -\gamma_{i}\cdot G_{i}(\mu_{i},\bm{\mu}_{-i})\geq 0 \quad \quad (\theta_{R,i})\\
    & \quad  G_{i}(\mu_{i},\bm{\mu}_{-i})\leq \budget_{i} \quad \quad (\theta_{B,i}),
\end{align}
where $(\theta_{B,i},\theta_{R,i})$ are the dual variables corresponding to the budget and ROI constraints.

\begin{definition}[Generalized Nash Equilibrium]
We call $\bm{\mu}^{*} \in \mathcal{A}^{N}$ a generalized Nash Equilibrium (GNE) if for any $i \in [N]$,  $\mu_{i}^{*} = \arg\max_{\mu_{i} \in  \feasible_{i}(\bm{\mu}_{-i})} F_{i}(\mu_{i},\bm{\mu}_{-i}^{*})$. For the set of objectives $\bm{F} = (F_{1} \dots F_{K})$, denote $\GNE(\bm{F})$ as the set of all GNEs.
\end{definition}


\begin{assumption}(Convex program)
\label{assum:convexprogram}
Assume for all $i \in [N]$, $ G_{i}(\bm{\mu})$ is convex in $\bm{\mu}$ and both $F_{i}(\bm{\mu})$  and  $F_{i}(\bm{\mu}) - \gamma_{i}G_{i}(\bm{\mu})$ are concave in $\bm{\mu}$ on $[0,\Bar{\mu}_{i}]$ for some $\Bar{\mu}_{i} < \infty$.
\end{assumption}

\begin{theorem}[POA]
Assume there are no ROI constraints i.e. $\gamma_{i}=0$ for all $i\in[N]$. Then under Assumption \ref{assum:convexprogram}, we have
\begin{align}
    \inf_{\bm{F}\in \mathcal{F}, \bm{\mu} \in \GNE(\bm{F})} \frac{\sum_{i\in[N]}F_{i}(\bm{\mu})}{\max_{\bm{\mu} \in \mathcal{C}}\sum_{i\in[N]}F_{i}(\bm{\mu})} =  \inf_{\bm{F}\in \lin, \bm{\mu} \in \GNE(\bm{F})} \frac{\sum_{i\in[N]}F_{i}(\bm{\mu})}{\max_{\mu \in \mathcal{C}}\sum_{i\in[N]}F_{i}(\bm{\mu})}
\end{align}
\end{theorem}
The LHS gives us an upper bound for POA, and this upper bound can be obtained by restricting ourselves to linear $\bm{F}$'s.

\begin{theorem}[POS]
Under Assumption \ref{assum:convexprogram}, there exists a function $f(\bm{\mu}) = \sum_{i\in[N]}F_{i}(\bm{\mu})$ such that $\nabla_{i}f = -\nabla_{i}F_{i}$
if and only if there exists continuously differentiable functions $\widetilde{\bm{F}} = (\widetilde{F}_{1}\dots \widetilde{F}_{N})$ where  $\widetilde{F}_{i}:\R^{N-1}\to \R$  such that for each $i\in [N]$,
\begin{align}
    F_{i}(\bm{\mu}) = \frac{\sum_{j\in[N]}\widetilde{F}_{j}(\bm{\mu}_{-j})}{N-1}- \widetilde{F}_{i}(\bm{\mu}_{-i}).
\end{align}
If such an $f$ exists, every $GNE$ is efficient.
\end{theorem}
% Efficiency of GNE
% (\cite{kulkarni2019efficiency})



\jason{Questions of interest:\\
1. When do GNEs exist?\\
2. What is the POA? How should we define POA in the first place?\\
3. Does boosting help improve welfare as in \cite{deng2021towards}? If so, by how much?\\
4. What is POS?\\
5. Given some properties/characteristics of $F_{i}$ and $G_{i}$, does there exist corresponding value distributions $P$?}


% \begin{proposition}
% When for all $i \in [N]$, $v_{i}$ is sampled from a uniform, exponential, or log-normal distribution, respectively, Assumption \ref{assum:convexprogram} holds.
% \end{proposition}


\begin{proposition}[Best response conditions]
\label{prop:bestreponse}
Under Assumption \ref{assum:convexprogram}, $\mu_{i}^{*} = \arg\max_{\mu \in  A_{i}(\bm{\mu}_{-i})\cap [0,\Bar{\mu}_{i}]} F_{i}(\mu_{i},\bm{\mu}_{-i})$ if and only if there exists $\theta_{B,i}^{*},\theta_{R,i}^{*} \geq 0$ such that
\begin{enumerate}
    \item $0 \in \partial  F_{i} (\mu_{i}^{*},\bm{\mu}_{-i}) +  \theta_{R,i}^{*}\partial \left(F_{i} - \gamma_{i}G_{i}\right)\left(\mu_{i}^{*},\bm{\mu}_{-i}\right)  + \theta_{B,i}^{*}\partial \left(-G_{i}\right)\left(\mu_{i}^{*},\bm{\mu}_{-i}\right)$
    \item $\theta_{B,i}^{*}
\left(\budget_{i} - G_{i}\left(\mu_{i}^{*},\bm{\mu}_{-i})\right)\right) = 0$
\item $ \theta_{R,i}^{*}\left(F_{i}(\mu_{i}^{*},\bm{\mu}_{-i}) - \gamma_{i} G_{i}(\mu_{i}^{*},\bm{\mu}_{-i})\right) = 0$
\end{enumerate}

\end{proposition}


\begin{example}[Uniform value distributions]
For the scenario with $N=2$ bidders, if $v_{i}\overset{i.i.d}{\sim} U([0,1])$, we have 
\begin{align}
& G_{i}(\bm{\mu}) = \I\left\{\mu_{-i} \leq \mu_{i}\right\}\frac{1+\mu_{-i}}{6(1+\mu_{i})^{2}} + \I\left\{\mu_{-i} > \mu_{i}\right\}\left(\frac{1}{2(1+\mu_{-i})} - \frac{1+\mu_{i}}{3(1+\mu_{-i})^{2}} \right)\\
& F_{i}(\bm{\mu}) =  \I\left\{\mu_{-i} \leq \mu_{i}\right\}\frac{1+\mu_{-i}}{3(1+\mu_{i})} + \I\left\{\mu_{-i} > \mu_{i}\right\}\left(\frac{1}{2}-\frac{(1+\mu_{i})^{2}}{6(1+\mu_{-i})^{2}}\right)\,.
\end{align}
Note that $ G_{i}(\bm{\mu}) $ is convex in $\mu_{i}$, and both $ G_{i}(\bm{\mu}) $ and $ F_{i}(\bm{\beta}) $ are differentiable everywhere in $\mu_{i}$.
Also both $F_{i}(\bm{\mu})$  and  $F_{i}(\bm{\mu}) - \gamma_{i}G_{i}(\bm{\mu})$ are concave in $\mu_{i}$ on $[0, \frac{1}{2}]$. Furthermore, the conditions in Proposition \ref{prop:bestreponse} become

\begin{enumerate}
    \item 
    \begin{align}
        0 = & \I\left\{\mu_{-i} \leq \mu_{i}\right\}\frac{1+\mu_{-i}}{3(1+\mu_{i})^{2}}\left(1 + \theta_{R,i}^{*} - \frac{1+\gamma_{i}\theta_{R,i}^{*}  + \theta_{B,i}^{*} }{1+\mu_{i}}\right)\\
    &  + \I\left\{\mu_{-i} > \mu_{i}\right\} \frac{1}{3(1+\mu_{-i})^{2}} \left((1+\mu_{i})(1 + \theta_{R,i}^{*}) -
    \left(1+\gamma_{i}\theta_{R,i}^{*}  + \theta_{B,i}^{*}\right)\right) 
    \end{align}
    \item $\theta_{B,i}^{*}
\left(\budget_{i} - G_{i}\left(\mu_{i}^{*},\bm{\mu}_{-i})\right)\right) = 0$
\item $ \theta_{R,i}^{*}\left(F_{i}(\mu_{i}^{*},\bm{\mu}_{-i}) - \gamma_{i} G_{i}(\mu_{i}^{*},\bm{\mu}_{-i})\right) = 0$
\end{enumerate}
\end{example}

\newpage
\section{POA for general outcomes with multiplier bound}
% Consider the following instance with 2 auctions and 2 bidders, where the multipliers $\alpha_{1},\alpha_{2} \in [L,U]$ for some $1\leq L\leq U < \infty$ such that $L^2 < U \leq L+1$: 
% % \setlength{\extrarowheight}{10pt}%
% \renewcommand{\arraystretch}{2}
% \begin{center}
% \begin{tabular}{|c | c c |} 
%  \hline
%   & A1 & A2  \\
%  \hline\hline
%  b1 & $1-\frac{d}{L}$ & 0 \\ 
%  \hline
%  b2 & $\frac{L}{U} - \frac{d}{L} + \epsilon $ & $\frac{d}{L}$  \\
%  \hline
% \end{tabular}
% \end{center}
% The parameter $d$ satisfies:
% \begin{align}
%     L\left(1-\frac{1}{U}\right) \leq d \leq \frac{L^2}{U}
% \end{align}
% where the second inequality guarantees b2's value in A1 is positive, and  $L\left(1-\frac{1}{U}\right) \leq \frac{L^2}{U} $ holds due to our assumption $U \leq L+1$. In this instance, there can only be 2 outcomes:
% \begin{itemize}
%     \item b1 wins A1 and b2 wins A2. Here, welfare equals 1 and is optimal. This outcome can be achieved by having identical multipliers $\alpha_{1} = \alpha_{2} = L$: for $b2$, payment is always 0, so b2's ROI constraint is satisfied. In this case, b1's margin is
%     \begin{align}
%         1-\frac{d}{L} - L\cdot \left(\frac{L}{U} - \frac{d}{L} + \epsilon\right) = 1- \frac{L^2}{U} + d(1-\frac{1}{L})-  \epsilon L \geq 0
%     \end{align}
%     where in the final inequality we used $U > L^2$, $L\geq 1 $ and $\epsilon$ small, so b1's ROI constraint is also satisfied.
%     \item b2 wins both A1 and A2. Here, welfare equals $\frac{L}{U} + \epsilon$. This outcome can be achieved by considering $(\alpha_{1},\alpha_{2}) = (L,U)$, during which the effective bid for b1 in A1 is $L-d$, and the effective bid for b2 is A1 is $L - \frac{U}{L}d  + \epsilon U \geq L-d + \epsilon U$.  In this case, b2's ``margin'' is 
%     \begin{align}
%       \left( \frac{L}{U} - \frac{d}{L} + \epsilon \right) +\frac{d}{L} -  L\cdot\left(1-\frac{d}{L}\right) = d - L\left(1-\frac{1}{U}\right) + \epsilon > 0
%     \end{align}
%     Hence b2's ROI constraint is satisfied.
% \end{itemize}  
% Therefore, in this instance, POA is $\frac{L}{U}$ by taking $\epsilon \to 0$. 

Consider the following instance with 2 auctions and 2 bidders, where the multipliers $\alpha_{1},\alpha_{2} \in [L,U]$ for some $1\leq L\leq U < \infty$ such that $L^2 < M := \min\{U,L+1\}$ and $U >L(LM-L^{2}+1)$: 
% \setlength{\extrarowheight}{10pt}%
\renewcommand{\arraystretch}{2}
\begin{center}
\begin{tabular}{|c | c c |} 
 \hline
  & A1 & A2  \\
 \hline\hline
 b1 & $(LM - L^{2}+1)x$ & 0 \\ 
 \hline
 b2 & $x$ & $(L^{2} - 1)x$  \\
 \hline
\end{tabular}
\end{center}
where $x > 0$. It is not difficult to see
$(LM - L^{2}+1)x > x$, so the optimal welfare is $(LM - L^{2}+1)x + (L^{2}-1)x = MLx$
In this instance, there can only be 2 outcomes:
\begin{itemize}
    \item b1 wins A1 and b2 wins A2. Here, welfare equals $MLx$ and is optimal. This outcome can be achieved by having identical multipliers $\alpha_{1} = \alpha_{2} = L$: for b2, payment is always 0, so b2's ROI constraint is satisfied. In this case, b1's margin is
    \begin{align}
       (LM - L^{2}+1)x - Lx = L(M-1)x - (L^{2}-1)x \geq  (M-1)x - (L^{2}-1)x > 0
    \end{align}
    where in the final inequality we used $M > L^2\geq L\geq 1$, so b2's ROI constraint is also satisfied.
    \item b2 wins both A1 and A2. Here, welfare equals $L^2x$. This outcome can be achieved by considering $(\alpha_{1},\alpha_{2}) = (L,U)$, during which the effective bid for b1 in A1 is $(LM - L^{2}+1)Lx$, and the effective bid for b2 is A1 is $Ux$, so b2 wins because by definition $U >L(LM-L^{2}+1)$. In this case, b2's ``margin'' is 
    \begin{align}
       x + (L^{2}-1)x - (LM - L^{2}+1)x
    \end{align}
    Hence b2's ROI constraint is satisfied.
\end{itemize}  
Therefore, in this instance, POA is $\frac{L^2x}{MLx} = \frac{L}{M}$. 


\newpage 
\section{POS for Nash Equilibrium (NE) with no multiplier bound}

Consider the following instance with 3 auctions and 2 bidders, where $0 < \delta < \epsilon < 1$: 
% \setlength{\extrarowheight}{10pt}%
\renewcommand{\arraystretch}{2}
\begin{center}
\begin{tabular}{|c | c c c|} 
 \hline
  & A1 & A2 & A3 \\
 \hline\hline
 b1 & $\epsilon$ & 1 & $\frac{1+\delta}{\delta \epsilon} - (1+\epsilon)$\\ 
 \hline
 b2 & 1 & $\delta$ & 0  \\
 \hline
\end{tabular}
\end{center}
It is not difficult to see that there can only be 2 possible outcomes: (O1) b1 wins A1, A2, A3; and (O2) b1 wins A2, A3 while b2 wins A1. Note that (O2) is the efficient outcome.

\textbf{Nonexistence of NE for (O2).} We first argue by contradiction that there exists no NE for outcome (O2), i.e. there is no efficient NE. Assume there exits a NE multiplier profile $ (\alpha_{1},\alpha_{2}) \in [1,\infty)^2$ that achieves (O2). Since b2's ROI constraint is satisfied, we have
\begin{align}
\label{eq:POSex1_1}
    1 > \alpha_{1}\epsilon
\end{align}
Next, since b1 has no incentive to deviate (to win auction A1), we have 
\begin{align}
\label{eq:POSex1_2}
    \epsilon + 1 + \frac{1+\delta}{\delta \epsilon} - (1+\epsilon) < \alpha_{2}(1+\delta)
\end{align}
This is because if the above equation does not hold, b1 can deviate to win A1, while maintaining  ROI constraint satisfaction. Moreover, since b1 wins A2, we have
\begin{align}
\label{eq:POSex1_3}
    \alpha_{2}\delta < \alpha_{1}
\end{align}
Finally, combining Eq (\ref{eq:POSex1_1}),(\ref{eq:POSex1_2}) and (\ref{eq:POSex1_3}), we get
\begin{align}
    \frac{1+\delta}{\delta \epsilon} < \alpha_{2}(1+\delta) < \frac{1+\delta}{\delta}\alpha_{1} < \frac{1+\delta}{\delta \epsilon} 
\end{align}
which is a contradiction. Hence there does not exist an NE that achieves (O2), i.e. there is no efficient NE. 

\textbf{Existence of NE for (O1).} We now argue $\alpha_{1} > \frac{1}{\epsilon}$ and $\alpha_{2} = 1$ is an NE that leads to (O1), i.e. b1 wins all auctions. Apparently, there is no incentive for b1 to deviate since she wins all auctions, and her ROI is satisfied, since $\frac{1+\delta}{\delta\epsilon} > 1+\delta$. Also, b2 has no incentive to deviate, because if she deviates to win only A1 (and not A2),  her margin is $1 - \alpha_{1}\epsilon < 0 $ since $\alpha_{1} > \frac{1}{\epsilon}$; and if she deviates to win both A1 and A2,  her margin is $1 + \delta - \alpha_{1}(\epsilon + 1) < 1 + \delta - (\epsilon + 1) < 0$.
 
 
From the above, we know that all NEs achieve the non-efficient outcome (O1), so all NEs have a POS of 
\begin{align}
    POS(\epsilon,\delta) = \frac{\frac{1+\delta}{\delta \epsilon}}{{\frac{1+\delta}{\delta \epsilon}} + 1-\epsilon} = \frac{1+\delta}{1+(\epsilon-\epsilon^2 +1)\delta}
\end{align}
Therefore, 
\begin{align}
   \min_{\epsilon\in (0,1), \delta \in (0,\epsilon)} POS(\epsilon,\delta) = \min_{\epsilon \in (0,1)} \frac{1+\epsilon}{1+(\epsilon-\epsilon^2 +1)\epsilon} \approx 0.917
\end{align}
where the final approximation takes  $\epsilon = \frac{\sqrt{5}-1}{2}$.

==> Scratch2_4_impossible.tex <==
Having presented a fairness guarantee in the previous Section \ref{sec:VCG} that improves according to the platform's ML advice accuracy, a natural question is that for a given level of accuracy $\beta$, \jason{can one achieve a universally better fairness guarantee than that of} Theorem \ref{thm:fairnessbound} via considering auction formats other than VCG? In this section, we demonstrate that the answer is negative when we restrict the auction to \jason{a broad class of truthful mechanisms (possibly randomized) with anonymous allocations. Here, we again emphasize that truthfulness is w.r.t. quasi-linear utility maximizers, and for bidders who have constraints or do not maximize quasi-linear utility e.g. autobidders whose objectives are defined in Equation (\ref{eq:autobidderprob}), truthful bidding may no longer be a dominant strategy in truthful auctions.} {\color{red} could we define the truthful notion somewhere formally? This can be confusing because when bidders have constraints (as they do in this work), VCG is no longer truthful.} To show this result, our strategy is to construct an autobidding instance with any auction format that belongs to  the aforementioned class of mechanisms, and argue that there is at least a bidder $i$ who will incur a welfare loss at least $\frac{1-\beta}{\alpha_{i}-1}\opt_{-i}$, which is the welfare loss upper bound shown in Theorem \ref{thm:fairnessbound}. 

The class of possibly randomized truthful mechanisms with anonymous allocations is extremely large, and therefore
to construct a suitable autobidding instance, we will rely on several simple yet fundamental definitions and properties for such class of auctions. Note that these properties are standard; see e.g. \cite{mehta2022auction}.
\begin{definition}[Allocation-anonymous auctions]
Consider any auction mechanism $\mathcal{M}$ whose (possibly random) allocation $\mathcal{X}:\R^{N}\to \R^{N}$ satisfies $\sum_{i\in[N]}\mathcal{X}_{i}(\bm{b}) \leq 1$ for any number of bidders $N$ and bid profile $\bm{b} \in \R_{\geq 0}^{N}/\{\bm{0}\}$. Then we say $\mathcal{M}$ is allocation-anonymous if the outcome for a permutation of any bid profile $\bm{b}$ is the permutation of the outcome for $\bm{b}$, i.e. for any permutation $\sigma: [N]\to [N]$, then $\left[\mathcal{X}(b_{\sigma(1), \dots \sigma(N)})\right]_{i} = \left[\mathcal{X}(\bm{b})\right]_{\sigma(i)} $ for any $i \in [N]$.
\end{definition}

\begin{remark}
\label{rem:anonymous}
\jason{An alternative view for auction anonymity is that the auction's allocation is  independent of individual bidders' identities. Mathematically, this says that for any set of bid values $\mathcal{B} =\{b_{1}\dots b_{K}\}$, there exists probabilities $\bm{q}(\bm{b})=(q_{0}(\bm{b}),q_{1}(\bm{b}) \dots q_{K}(\bm{b})) \in [0,1]^{K+1}$ where $q_{k}(\bm{b}) = \prob(\text{bid value $b_{k}$ wins auction $\mathcal{M}$ given competing bids $\bm{b}_{-k}$})$ only depends on the bid values $\bm{b}$.}
\end{remark}
The following technical definition and lemma (i.e. Definition \ref{def:monop} and Lemma \ref{lem:singlebiddercost}) concerns the scenario where only one bidder participates in the auction (others bid 0), and present an upper bound on the probability and cost  respectively for the single bidder to win the auction. {\color{red} NG: Let's say why we care about this scenario.}
\begin{definition}[Single bidder purchase probability and bid threshold]
\label{def:monop}
For any allocation-anonymous and truthful auction $\mathcal{M}$, consider the setting with a single bidder. Let $b > 0$ be the submitted bid, and define 
\begin{align}
    \pi_{\mathcal{M}} = \lim_{b\to \infty}\prob(\text{bidder wins item with bid $b$})\,,
\end{align}
where the limit exists because in a truthful auction, $\prob(\text{bidder wins item with bid $b$})$ increases in $b$. {\color{red} again, if we define truthfulness formally, we can mention this ``$\prob(\text{bidder wins item with bid $b$})$ increases in $b$" there. } Assume this max probability is reached at some bid threshold $Q_{\mathcal{M}}$, i.e.
\begin{align}
   Q_{\mathcal{M}} = \min\left\{b>0: \prob(\text{bidder wins item with bid $b$}) =  \pi_{\mathcal{M}}\right\} \,.
\end{align}
\end{definition}
Note that in a deterministic single-slot auction that allocates to the highest bidder,  $\pi_{\mathcal{M}} = 1$, and $Q_{\mathcal{M}}  \to 0$. For example, in an SPA {\color{red} maybe highlight the fact that you are talking about SPA with no reserve.}, the single bidder can win the auction with any arbitrarily small positive bid with probability 1. {\color{red} could we have other examples that do not lead to a trivial value for $Q_{\mathcal M}$?}
\begin{lemma}[Lemma 4 in \cite{mehta2022auction}]
\label{lem:singlebiddercost}
For any allocation-anonymous and truthful auction $\mathcal{M}$ with single-bidder purchase probability $ \pi_{\mathcal{M}}$ and bid threshold $ Q_{\mathcal{M}}$, the expected cost for a single bidder for winning the item is at most $\pi_{\mathcal{M}} \cdot Q_{\mathcal{M}}$.
\end{lemma}

{\color{red} NG: up to here, it is still not clear why we are talking about the single bidder case and Lemma 4 in Mehta 2022. Shall we start with presenting Theorem 6?}

Our main result for this section is the following Theorem \ref{thm:imposs}, where we present an autobidding instance w.r.t. to any allocation-anonymous, truthful, and possibly randomized auction in which there must exist a bidder $i$ who will incur a welfare loss at least $\frac{1-\beta}{\alpha_{i}-1}\opt_{-i}$, which is the welfare loss upper bound in Theorem \ref{thm:fairnessbound}. 
\begin{theorem}
\label{thm:imposs}
For any auction $\mathcal{M}$ {\color{red} didn't we use ``$A$" to denote auctions?} that is allocation-anonymous, truthful, and possibly randomized, consider an autobidding problem instance w.r.t.  $\mathcal{M}$ with $M = 2K+1$ auctions and $N = K+1$ bidders. Fix bidder 0's {\color{red}NG: when we index the bidders, did we start from $0$? I think we did not use $0$.} bid multiplier to be $\alpha_{0}$ and some $\beta\in [0,1)$. Consider the bidder values $\{v_{i,j}\}_{i\in[N],j\in[M]}$ given in the following table. {\color{red} again, we can have a cleaner theorem by just stating the result (not the instance). We can then discuss the instance in a proof sketch. The proof sketch should provide some insights as the instance looks complicated. At least, I did not digest how the example is constructed.}
\renewcommand{\arraystretch}{2}
\begin{center}
\begin{tabular}{|c | c c c c c c c c c|} 
 \hline
  & $A_{1}$ & $A_{2}$ & \dots  &   $A_{K}$  & $A_{K+1}$ & $A_{K+2}$ & \dots & $A_{2K}$ &  $A_{2K+1}$\\
 \hline\hline
 bidder 0 & $v$ & $v$ & \dots & $v$ & 0 & 0 & \dots & 0  & $X$\\ 
 \hline
bidder 1  & $\frac{\alpha_{0}v+\epsilon}{\rho}$ & $\frac{\alpha_{0}v+2\epsilon}{\rho}$  & \dots &  $\frac{\alpha_{0}v+K\epsilon}{\rho}$ & $\gamma$  & 0 &  \dots & 0 & 0\\
  \hline
 bidder 2  & $\frac{\alpha_{0}v+2\epsilon}{\rho}$ & $\frac{\alpha_{0}v+3\epsilon}{\rho}$  & \dots &  $\frac{\alpha_{0}v+\epsilon}{\rho}$ & 0 &  $\gamma$ & \dots &  0 & 0  \\
 \hline
 \vdots & \vdots &  \vdots  &  &   \vdots  &  \vdots & \vdots & & \vdots & \vdots \\
  \hline
bidder $K$  & $\frac{\alpha_{0}v+K\epsilon}{\rho}$ & $\frac{\alpha_{0}v+\epsilon}{\rho}$  & \dots &  $\frac{\alpha_{0}v+(K-1)\epsilon}{\rho}$ & 0  & 0  & \dots & $\gamma$ & 0\\
   \hline
%   \hline
%   Reserve & $\beta v$ & $\beta v$  & \dots & $\beta v$  & $\beta \gamma$ &  $\beta \gamma$ & \dots &  $\beta \gamma$ & $\beta X$\\
%   \hline
\end{tabular}
\end{center}
In the table, we let $\gamma > \frac{Q_{\mathcal{M}}}{\beta} > Q_{\mathcal{M}}$, $\epsilon = O(1/K^{3})$ and $v = \frac{1-\beta}{\alpha_{0}-1}\cdot \pi_{\mathcal{M}}\cdot \gamma$. Let $\rho,X$ {\color{red} instead of $X$, you can use $y$ for instance.} and a large enough $K$ satisfy the following:
\begin{align}
\begin{aligned}
\label{eq:imposs:params}
%   & \gamma \geq \max\left\{\frac{1}{(1-\beta)\pi_{\mathcal{M}}}\left( \frac{(1-\beta)\alpha_{0}}{\alpha_{0}-1} + \frac{(K+1)K}{2}\epsilon\right),\frac{Q_{\mathcal{M}}}{\beta} \right\}\\ 
   & \alpha_{0}<\rho <\frac{\alpha_{0}}{\beta} ~\text{s.t.}~\frac{\alpha_{0}v+K\epsilon}{\rho} < v,\quad \text{ and } X > \max\left\{\frac{Q_{\mathcal{M}}}{\alpha_{0}}, \frac{\alpha_{0}v}{\pi_{\mathcal{M}}}\right\}\,.
  \end{aligned}
\end{align}
Further, suppose the platform enforces personalized reference prices $\bm{r}\in \R_{\geq 0}^{N\times M}$ on top of auction $\mathcal{M}$, where $r_{i,j} = \beta v_{i,j}$.
 Then, letting the (possibly random) outcome be $\bm{x}$ when bidders 1, ... K all adopt the bid multiplier $\rho$, 
 the ROAS constraints for all bidders are satisfied when $K\to\infty$ and $\rho \to \alpha_{0}$, and for bidder $0$ we have 
 \begin{align}
    \lim_{K\to \infty} \frac{\E_{\mathcal{M}}[\loss_{0}(\bm{x})]}{\E_{\mathcal{M}}\left[\opt_{-0}\right]} \geq \frac{1-\beta}{\alpha_{0}-1}\,,
 \end{align}
 where $\E_{\mathcal{M}}$ is taken w.r.t. the randomness in outcome $\bm{x}$ due to randomness in the auction $\mathcal{M}$, and the loss of bidder 0, namely $\loss_{0}$, is defined in Equations (\ref{eq:loss}).
%  fairness guarantee is at most $1-\frac{1-\beta}{\alpha_{0}-1}\cdot \frac{\opt_{-0}}{\opt_{0}}$.
\end{theorem}
\begin{remark}
\label{rem:retainanonym}
\jason{
Generally speaking, enforcing personalized reserve prices to an allocation-anonymous auction would invalidate allocation-anonymity. However, for every auction $j \in [K]$ within the autobidding instance in Theorem \ref{thm:imposs}, a bid from any bidder resulting from uniform bidding with multiplier at least 1 would always be greater than the reserve price of the bidder: for any auction $j \in [K]$, any submitted bid $b$ (independent of bidder) satisfies $b \geq \min_{i=0...K+1} v_{i,j} > \frac{\alpha_{0}v}{\rho} \overset{(a)}{>} \beta v  \overset{(b)}{=}\max_{i=0...K} r_{i,j}$ where both (a) and (b) follow from Equation (\ref{eq:imposs:params}). Therefore, the outcome when enforcing  personalized reserves is the same as that of not having reserves, conditioned on uniform bidding with multiplier at least 1. Therefore, in the sense of Remark \ref{rem:anonymous}, for each auction $j \in [K]$ and for bid values $\bm{b}$ that arise from uniform bidding with multiplier at least 1, there exists probabilities $\bm{q}(\bm{b})=(q_{0}(\bm{b}),q_{1}(\bm{b}) \dots q_{K}(\bm{b})) \in [0,1]^{K+1}$ where $q_{k}(\bm{b}) = \prob(\text{bid value $b_{k}$ wins auction $\mathcal{M}$ given competing bids $\bm{b}_{-k}$})$ only depends on the bid values $\bm{b}$ and is independent of bidder identity.} {\color{red}  I am not sure if this is the best place for this remark. Also, this is quite confusing as we were saying VCG is the best among all anonymous and truthful mechanisms. Now, we are saying VCG does not even belong to this class. On a related note, for any truthful auction $A$, could we define some other truthful auction $A'$ with reserve prices? If yes, could we say $A'$ is  anonymous if its allocation rule only depends on submitted bids and reserve prices. That is, when we swap the identity of two bidders, we swap their bids, as well as,  their reserve prices. Finally, I did not fully follow this  remark. Are we saying VCG is anonymous only when $\alpha_i$'s are one? If yes, this does not seem to be enough. }
\end{remark}

The proof of Theorem \ref{thm:imposs} is presented in Appendix \ref{pf:thm:imposs}.  VCG is also truthful and allocation-anonymous, 
Theorem \ref{thm:imposs} along with Theorem \ref{thm:fairnessbound} implies that with $\beta$-accurate ML advice, VCG achieves the best possible fairness guarantee among the broad class of allocation-anonymous, truthful and possibly randomized auctions.




==> Scratch2_model.tex <==
Consider a platform running an autobidding instance $\inst = ( N,M,\mathcal{A},\bm{r},\bm{v})$ where there are $N$ bidders bidding in $M$ parallel position auctions \cite{lahaie2007sponsored,varian2007position} of the format $\mathcal{A}$ (e.g. VCG, GSP, GFP etc.) that are labeled $A_{1}\dots A_{M}$. Here, $\bm{r} = (r_{i,j})\in\R_{\geq 0}^{N\times M} $, where $r_{i,j}$ is the reserve price for bidder $i \in [N]$ in auction $A_{j}$; and $\bm{v} = (v_{i,j})\in\R_{\geq 0}^{N\times M}$ where $v_{i,j}$  is the value of bidder $i$ in auction $j$.  We assume for simplicity that no pair of bidders have the same value in an auction, i.e.  $v_{i,j}\neq v_{i',j}$ for any any two bidders $i\neq i'$ and any $j\in[M]$. {\color{red} need to justify this assumption. Is this a crucial assumption or do we make it to ease the technical analysis?} In each auction $j$, let there be $\numslot_{j}$ available positions associated with position discounts $\mu_{j}(\ell)$ for the $\ell$'th position.  {\color{red} the notion of ``position discount" needs to be defined. If you'll define it later, you can say it here.} Here assume for 
any auction $j \in [M]$, we have $1\geq \mu_{j}(1) > \mu_{j}(2)>  \dots> \mu_{j}(\numslot_{j}) > 0 $, and without loss of generality, we set   $\mu_{j}(\numslot_{j}+1) =\ldots = \mu_{j}(N) =0$. {\color{red} you can also say positions with lower indices are more visible and have higher position discounts. }








\subsection{Auction outcomes, efficiency, welfare guarantees and fairness}
\jason{The platform solicits bids from bidders $\bm{b}=(b_{i,j})_{i\in[N],j\in[M]} \in \R_{\geq 0}^{N\times M}$, where $b_{i,j}$ is the bid from bidder $i$ in auction $j$. Then, it ranks bidders by their bids in each auction (tie-breaking by bidder indices) and allocates the $\ell$th slot/position of an auction to the bidder with the $\ell$th highest bid in that auction. We refer to these rankings over all auctions as the \textit{outcome} of the autobidding instance,  defined as} $\bm{x} = (\bm{x}_{1},\ldots, \bm{x}_{M})$ where $\bm{x}_{j} = (x_{i,j,\ell})_{i\in[N],\ell \in [\numslot_{j}]}\in \{0,1\}^{N\times \numslot_{j}}$ is the outcome vector in auction $j$ and further $x_{i,j,\ell} = 1$ if bidder $i$ won position $\ell$ in auction $j$ and 0 otherwise. Note that each bidder $i$ can win at most one position in an auction $j$, i.e. $\sum_{\ell\in [\numslot_{j}]}x_{i,j,\ell} =1 $.

\yuan{Shall we also mention each position can be allocated to at most one bidder in expectation?}

\jason{For any outcome $\bm{x}$, let $\ell_{i,j}$ be the position of bidder $i$ in auction $j$, and define $\well_{i,j}(\bm{x}) = \mu_{j}(\ell_{i,j})\cdot v_{i,j} x_{i,j,\ell}$  as bidder $i$'s acquired welfare in auction $j$.} {\color{red}$\ell_{i,j}$ is not well defined when bidder $i$ is not assigned any slot in auction $j$.} The welfare contribution of bidder $i$ is then defined as $\well_{i}(\bm{x}) = \sum_{j\in[M]} \well_{i,j}(\bm{x})$, and the total welfare of outcome $\bm{x}$ is $\well(\bm{x}) =\sum_{i\in[N]} \well_{i}(\bm{x})$.  Further, let $\ell_{i,j}^{\opt}$ be the position of bidder $i$ in auction $j$ when ranked according to true values $\bm{v} \in \R_{\geq 0}^{N\times M}$. Then we call the outcome $\bm{x}^{\opt}$ with $x_{i,j,\ell}^{\opt} = \I\{\ell = \ell_{i,j}^{\opt}\}$, the \textit{efficient outcome}. Note that $\bm{x}^{\opt}$ is called efficient because it yields the largest total welfare, i.e. $\bm{x}^{\opt} = \arg\max_{\bm{x}} \well(\bm{x})$. Similarly, let $\opt_{i,j}= \mu_{j}(\ell_{i,j}^{\opt})\cdot v_{i,j}$, $\opt_{i}(\bm{x}) = \sum_{j\in[M]} \opt_{i,j}(\bm{x})$, and $\opt(\bm{x}) =\sum_{i\in[N]} \opt_{i}(\bm{x})$ be the welfare of bidder $i$ in auction $j$, total welfare contribution of bidder $i$, and total welfare, respectively, under the  efficient outcome.  Finally,  we denote $\feas$
as the set of all feasible outcomes where every bidder's ROI constraint {\color{red} where did you define ROI constraint? This should be defined formally first.} is satisfied. 



Our goal is to present a characterization for how model primitives of the autobidding instance $\inst$ impact overall fairness of bidders defined as followed:
\begin{definition}[$\delta$-fairness]
\label{def:fairness}
For any $\delta \in [0,1]$, an autobidding instance is $\delta$-fair for bidder $i$ if 
% $ \min_{\bm{x}\in \feas}\frac{\well_{i}(\bm{x})}{\opt_{i}}~\geq~ \delta$
\begin{align*}
    \min_{\bm{x}\in \feas}\frac{\well_{i}(\bm{x})}{\opt_{i}}~\geq~ \delta
\end{align*}
\end{definition}
Alternatively, in this paper we also consider the loss in welfare compared to a bidder's  welfare contribution under the efficient outcome, formally defined as followed:
\begin{definition}[Welfare loss w.r.t. efficient outcome]
\label{def:welfareloss}
For an outcome $\bm{x}$ and any bidder $i\in [N]$, let $\mathcal{L}_{i}(\bm{x}) = \{j\in [M]: \well_{i,j}(\bm{x})< \opt_{i,j}\}$ be the set of auctions in which bidder $i$'s acquired welfare is less than that of her welfare under the efficient outcome. Then, we define the loss of bidder $i$ under outcome $\bm{x}$ w.r.t. the efficient outcome $\bm{x}^{\opt}$ (or simply ``welfare loss'' in the rest of the paper):
\begin{align}
\label{eq:loss}
\loss_{i}(\bm{x}) = \sum_{j \in \mathcal{L}_{i}(\bm{x})}\left(\opt_{i,j}-\well_{i,j}(\bm{x})\right)\,.
\end{align}
\end{definition}
\begin{remark}
\label{rem:rewritebadauctions}
For any outcome $\bm{x}$, let $\ell_{i,j}$ be the position (i.e. ranking) of bidder $i$ in auction $j$, and recall that $\ell_{i,j}^{\opt}$ is the position of bidder $i$ in auction $j$ under the efficient outcome $\bm{x}^{\opt}$. Then, set $\mathcal{L}_{i}(\bm{x}) = \{j\in [M]: \well_{i,j}(\bm{x})< \opt_{i,j}\}$ can also be interpreted as the set of auctions where bidder $i$'s ranking under $\bm{x}$ is lower than her ranking $\bm{x}^{\opt}$, or in other words the set of auctions that incur a welfare loss w.r.t. $\bm{x}^{\opt}$. Hence we can also rewrite $\mathcal{L}_{i}(\bm{x}) = \{j\in[M]: \ell_{i,j} > \ell_{i,j}^{\opt}\}$.
\end{remark}


\begin{remark}
\label{rem:SPAinterpret}
In the special case where there is only a single slot in each auction, i.e. $\numslot_{j}=1$ for all $j \in [M]$, we simplify notation as followed: let $v_{j}^{+} = \max_{i\in[N]}v_{i,j}$ be the largest value in auction $j$, and $\bm{x}\in\{0,1\}^{N\times M}$ denote an auction outcome, where $x_{i,j} = 1$ if bidder $i$ won auction $j$ and 0 otherwise. Then for outcome $\bm{x}$, the set $\mathcal{L}_{i}(\bm{x}) = \{j\in [M]: v_{i,j} = v_{j}^{+} \text{ but } x_{i,j} = 0\}$ is the set of auctions in which $i$ has the largest value but did not win,  and her loss is $\loss_{i}(\bm{x}) = \sum_{j\in \mathcal{L}_{i}(\bm{x})}v_{i,j}$.
\end{remark}

The following proposition connects the notion of welfare loss (as in  \ref{def:welfareloss}) and fairness (as in Definitions \ref{def:fairness}). The proposition shows that  an upper bound on  welfare loss can be directly translated into a welfare lower bound that corresponds to our fairness notion.
\begin{proposition}[Translating loss to fairness]
\label{prop:boundloss}
Assume for bidder $i \in [N]$ and outcome $\bm{x}$ we have $\loss_{i}(\bm{x})\leq B$ for some $B > 0$. Then, $\frac{\well_{i}(\bm{x})}{\opt_{i}}\geq 1- \frac{B}{\opt_{i}}$.
\end{proposition}
\textit{Proof}. For simplicity, denote $\delta_{i,j}= \opt_{i,j}-\well_{i,j}(\bm{x})$. Then, $\opt_{i}-\well_{i}(\bm{x}) = 
\sum_{j\in [M]:\delta_{i,j}>0}\delta_{i,j}  + \sum_{j\in [M]:\delta_{i,j}=0}\delta_{i,j} + \sum_{j\in [M]:\delta_{i,j}<0}\delta_{i,j} =
\loss_{i}(\bm{x}) + \sum_{j\in [M]:\well_{i,j}(\bm{x}) > \opt_{i,j}}\left(\opt_{i,j}-\well_{i,j}(\bm{x})\right) \leq \loss_{i}(\bm{x}) \leq B\,.$ Rearranging and dividing both sides by $\opt_{i}$ we get $\frac{\well_{i}(\bm{x})}{\opt_{i}}\geq 1- \frac{B}{\opt_{i}}.  \qedwhite$ 

\jason{Here we remark that it is possible to have $\well_{i,j}(\bm{x}) > \opt_{i,j}$ because bidders may overbid, and therefore win auctions/slots that they would not have won under the efficient outcome.} 

% \yuan{Since this is the first proof of the paper and it is actually a simple one, let's make it clear with more details so that the reviewer won't be struggling in reading this. In the first step, add one more equation to partition the auctions into three categories with $\well_{i,j}(\bm x)$ larger than, less than, and equal to $\opt_{i,j}$. And briefly explain why $\well_{i,j}(\bm x)$ can be larger than $\opt_{i,j}$ (since the bid multiplier could be larger than $1$).} 


% \begin{proof}\begin{align*}
%     \opt_{i}-\well_{i}(\bm{x}) = \loss_{i}(\bm{x}) + \sum_{j\in [M]:\well_{i,j}(\bm{x}) > \opt_{i,j}}\left(\opt_{i}-\well_{i}(\bm{x})\right) \leq \loss_{i}(\bm{x}) \leq B\,.
% \end{align*} 

% \end{proof}




\subsection{Objectives and behavior of autobidders}
\label{subsec:autobidder}
\jason{Once the platform solicits bids  $\bm{b}=(b_{i,j})_{i\in[N],n\in[M]} \in \R_{\geq 0}^{N\times M}$ from bidders and determines the corresponding outcome $\bm{x}(\bm{b})$ according to the parallel auctions' allocation rules (i.e. rank according to bids in each auction), the platform charges payment $\pay_{i,j}(\bm{b})$ to bidder $i$ for auction $j$ according pre-determined payment rules.}  \yuan{Usually, people write payment function depending on bids as well rather than allocation. You anyway need the bid information to compute payments. Maybe it is better to omit the dependence here as what we did in the NeurIPS paper. Actually, you did not write dependence in the following example as well...well, let's make it depend on the bids since you need it to define the autobidder's objective} For illustrative purposes, the following are examples of payment rules in several classic mutli-slot auction formats. \yuan{Maybe I missed it but have we defined allocation rule somewhere?} 

{\color{red} The allocation rule is defined earlier. But, I suggest we discuss allocation and payment rules next to each other. Also, the allocation rule we had before did not have reserve prices. It just said we allocate the $\ell$-th slot to the bidder with the $\ell$-highest bid. With reserve prices, this is no longer accurate. On a related note, we can have a subsection where we discuss the auction rules. This section was supposed to discuss bidders' behaviour and objective.}


\begin{example}[Example payment rules]
\label{ex:payment}
{\color{red} in position discounts, subscript $j$ is missing.}
Suppose bidders submit bids $\bm{b}=(b_{i,j}) \in \R_{\geq 0}^{N\times M}$, and each bidder $i$ is associated with a personalized reserve $r_{i,j}\in \R_{\geq 0}$ for auction $j$.
We denote $(\Hat{b}_{1,j}\dots \Hat{b}_{N,j})$ to be the bids' order statistics where $\Hat{b}_{\ell,j}$ is the $\ell$th largest bid in auction $j$. Then, for any bidder $i$ who won a slot $\ell_{i,j}\in [\numslot_{j}]$ in auction $j$, the following shows her corresponding payment $p_{i,j}$ under different auction formats: (1) VCG: $p_{i,j}^{\text{VCG}}(\bm{b}) = \sum_{\ell = \ell_{i,j}}^{\numslot_{j}}(\mu(\ell) - \mu(\ell+1))\cdot\max\{\Hat{b}_{\ell+1,j},r_{i,j}\}$; (2) GSP: $p_{i,j}^{\text{GSP}}(\bm{b}) =\mu(\ell_{i,j})\cdot \max\{\Hat{b}_{\ell_{i,j}+1},r_{i,j}\}$; (3) GFP: $p_{i,j}^{\text{GFP}}(\bm{b}) =\mu(\ell_{i,j})\cdot \max\{\Hat{b}_{\ell_{i,j}},r_{i,j}\}$. It is well known that for the same  bid profile $\bm{b}$, 
we have the following payment dominance relation: $p_{i,j}^{\text{GFP}}(\bm{b}) \geq p_{i,j}^{\text{GSP}}(\bm{b}) \geq p_{i,j}^{\text{VCG}}(\bm{b})$ for all $i\in[N]$ and $j\in[M]$ (see e.g. \cite{edelman2007internet}).

% \begin{align*}
%   &\textbf{VCG: }\sum_{\ell = \ell_{i,j}}^{\numslot_{j}}(\mu(\ell) - \mu(\ell+1))\max\{\Hat{b}_{\ell+1},r_{i,j}\},\quad  \textbf{GSP: } \mu(\ell_{i,j})\max\{\Hat{b}_{\ell_{i,j}+1},r_{i,j}\}\\ 
%   & \textbf{GFP: } \mu(\ell_{i,j})\mu(\ell_{i,j}) \max\{\Hat{b}_{\ell_{i,j}},r_{i,j}\}
% \end{align*}
     
% \begin{enumerate}
%     \item \textbf{VCG: } $p_{i,j} = \sum_{\ell = \ell_{i,j}}^{\numslot_{j}}(\mu(\ell) - \mu(\ell+1))\max\{\Hat{b}_{\ell+1},r_{i,j}\}$.
%      \item \textbf{GSP: } $p_{i,j} = \mu(\ell_{i,j})\max\{\Hat{b}_{\ell_{i,j}+1},r_{i,j}\}$.
%      \item \textbf{GFP: } $p_{i,j} = \mu(\ell_{i,j}) \max\{\Hat{b}_{\ell_{i,j}},r_{i,j}\}$.
% \end{enumerate}

\end{example}

We consider the setting where bidders aim to maximize total value over $M$ auctions, subject to a ROAS {\color{red} ROI or ROAS? Please recall what ROAS stands for.} constraint which guarantees total expenditure is less than total acquired value across all auctions. {\color{red} you can relate this to the ROI constraint with a certain value for the ROI target. Right? Is it crucial to consider ROAS, not ROI?} Mathematically, bidder $i$, when fixing other bidders' bids $\bm{b}_{-i}\in\R_{\geq 0}^{(N-1)\times M}$, decides on bids $\bm{b}_{i}\in \R_{\geq 0}^{M}$ for all $M$ auctions for the following optimization problem: 
\begin{align*}
    \max_{\bm{b}_{i}\in \R_{\geq 0}^{M}} ~\well_{i}(\bm{x}(\bm{b}_{i},\bm{b}_{-i})) \quad \text{s.t.}~ \well_{i}(\bm{x}(\bm{b}_{i},\bm{b}_{-i})) \geq \sum_{j\in[M]}p_{i,j}(\bm{b}_{i},\bm{b}_{-i})\,.
\end{align*}
It has been shown in previous literature \citep{aggarwal2019autobidding,deng2021towards,balseiro2021robust,mehta2022auction} that for truthful {\color{red} If truthfulness is important, you can discuss it when you introduce different auction formats.} (i.e. ex-post incentive compatible) auctions, the optimal bidding strategy for any autobidder $i$ is to submit bid values of the form $b_{i,j}= \alpha_{i}v_{i,j}$ for auction $j\in [M]$, where $\alpha_{i}>0$ is a bid multiplier that is used uniformly across all auctions. Such a bidding strategy is called \textit{uniform bidding}. Note that for autobidders, taking any uniform bid multiplier $\alpha_{i} <1$ is weakly dominated by setting $\alpha_{i}  = 1$. This is because by setting $\alpha_{i}  = 1$, the bidder can acquire larger total value as compared to setting $\alpha_{i} <1$. At the same time, 
the bidder bids truthfully in all auctions, and because the payment in any auction is no greater than the winning bid value in truthful auctions, the ROAS constraint is always satisfied under  $\alpha_{i}  = 1$. Therefore, we focus on undominated bid-multipliers, i.e.  $\alpha_{i} \in [1,\infty)$ for all $i \in [N]$. {\color{red} This is a bit confusing as GSP and GFP are not truthful. So, let's first clarify we  first investigate VCG which is truthful. The above discussion may wrongfully suggest you are saying all the three auctions are truthful.}

In light of the above discussion on uniform bidding, in the following Sections \ref{sec:VCG} and \ref{sec:imposs}, we address VCG auctions which are truthful, and hence only focus on uniform bidding strategies. Later in Section \ref{sec:extensions} when we extend our results to non-truthful auctions such as GSP and GFP, we will discuss more general bidding strategies, in particular, non-uniform bidding.
\section{Incorporating ML advice for bidder values as personalized reserve prices}
\label{sec:reserves}
With modern machine learning (ML) models and frameworks, 
online ad platforms can utilize available historical data (e.g. bid logs, keyword characteristics, user profiles, etc.) to produce predictive signals (or more generally ML advice) on autobidders' values. In this work, we specifically focus on ML advice that take the form of a \textit{lower-confidence bound} of true advertiser values.

Our key approach to incorporate this type of ML advice in our autobidding setting, is via simply setting personalized reserve prices to be the lower confidence bound for each bidder's value. To motivate this approach, consider the following example:
\begin{example}[Motivating example for ML advice as reserves]
\label{ex:motivate}
Consider 2 bidders competing in 2 second-price auctions (SPA) whose values are indicated in the following table with some $v > 0$ and small positive $\epsilon \to 0$.
\renewcommand{\arraystretch}{2}
\begin{center}
\begin{tabular}{|c | c c| } 
 \hline
  & Auction 1 & Auction 2   \\
 \hline\hline
 bidder 1 & $v$ & $\epsilon$ \\
 \hline
 bidder 2 & $\frac{v}{2}$  & $v$ \\
 \hline
\end{tabular}
\end{center}
\end{example}
For illustrative convenience suppose bidder 1 sets her bid multiplier to be $\alpha_{1} = 1$. Then when her competitor bidder 2 sets a multiplier $\alpha_{2} > 2$, bidder 2 will win both auctions and acquire a total value of $v_{2,1} + v_{2,2}=\frac{3}{2}v$ while submitting a payment of $\alpha_{1}(v_{1,1} + v_{1,2}) = v+\epsilon$. In this case, when $\epsilon\to 0$, bidder 2 satisfies her ROAS constraint and extracts all bidder 1's welfare, leaving her with no value. \jason{We also highlight that this bid mulitplier profile constitutes an equilibrium, because bidder 1 cannot raise her bid multiplier to outbid bidder 2 for auction 1, since with $\alpha_{2} > 2$ bidder 1 would violate her ROI constraint if she bid more than $\alpha_{2}v_{2,1} > v$.}  \yuan{Highlight that this is actually an equilibrium since bidder 1 cannot raise the bid to win Auction 1 without violating the ROAS constraint.}

Now suppose for each value $v_{i,j}$ ($i,j \in [2]$), the platform possesses a lower-confidence type of ML advice, namely $(\Hat{v}_{i,j}^{-})_{i,j\in[N]}$ such that $\beta v_{i,j}\leq\Hat{v}_{i,j}^{-} < v_{i,j}$ for some $\beta>\frac{1}{2}$, and sets personalized reserves $r_{i,j} = \Hat{v}_{i,j}^{-}$. If bidder 2 attempts to win both auctions by setting $\alpha_{2} > 2$, her payment will be at least  $\max\{\beta v_{1,1}, \alpha_{1} v_{1,1}\} +  \max\{\beta v_{1,2}, \alpha_{1} v_{1,2}\} = v + \beta v > \frac{3}{2}v$, which would violate her ROAS constraint. Therefore, via incorporating ML advice as personalized reserves, bidder 1's competitor is prohibited from outbidding her in auction 1, and hence safeguarding bidder 1's welfare.

\jason{The main observation from the above example is that without reserve prices, bidder 2 acquires a large margin for her ROAS constraint by winning auction 2 where competition is small and cost is low. Therefore, she can raise her bid to outbid bidder 1 in auction 1 without violating her overall ROAS constraint by compensating for the high cost in auction 1 with her acquired margin in auction 2. By setting personalized reserves properly, the platform can increase bidder 2's payment in auction 2, which  in turn decreases the manipulative power of bidder 2 by reducing the ROA margin she can acquire from auction 2.}

%  the platform can increase payments and in turn decrease the manipulative power of bidders who significantly raise bids to outbid competitors in certain auctions (i.e. auction 1) and compensate for the high expenditure with value acquired from auctions with small competition and low costs (i.e. auction 2). 
%  \yuan{This sentence is too long and hard to read. Rephrase: Observe that in our example, bidder 2 acquires a big margin in her ROAS constraint from auction 2 with small competition and low cost, and therefore, she is able to raise her bid to outbid bidder 1 in auction 1 without violating her overall ROAS constraint. By setting personalized reserves properly, the platform can increase bidder 2's payment in auction 2, which  in turn decrease the manipulative power of bidder by reducing her margin from auction 2.} 

\jason{We formally characterize reserves prices with which the platform can reduce bidders' manipulative power using the notion of \textit{approximate reserves} defined as followed.}
\begin{definition}[$\beta$-accurate ML advice and approximate reserves]
\label{def:reserve}
In an autobidding instance $\inst = ( N,M,\mathcal{A},\bm{r},\bm{v})$, suppose the platform possess a lower-confidence type of ML advice $(\Hat{v}_{i,j}^{-})_{i,j\in[N]}$. If 
$\Hat{v}_{i,j}^{-}  \in [\beta v_{i,j},v_{i,j})$ with some $\beta \in (0,1)$ for all $i,j$ and $v_{i,j}\neq 0$, we say that the ML advice is $\beta$-accurate.  Further, if the platform sets $r_{i,j} = \Hat{v}_{i,j}^{-}$, then we say that reserve prices $\bm{r}$ are $\beta$-approximate.
\end{definition}
The gap between the lower bound $\beta v_{i,j}$ and the true value $v_{i,j}$ represents the inaccuracies of the platform's ML advice. In other words, $\beta$ can be perceived as a quality measure of the platform's ML advice for advertiser value, such that larger $\beta$ represents better advice quality.  We point out that in many real-world settings, ML advice is presented as confidence intervals for true advertiser values. This can apparently be viewed as a special case of our required lower-confidence type of ML advice, as we show in the  following example for practical relevance:
% Note that the above inaccuracies are one-directional as we only impose a lower bound on true values. This is without loss of generality because for signals with two-sided bounded errors,one can simply set the approximate reserve to be the lower bound on the estimate. To illustrate this point, we present the following example that may be of practical relevant regarding how one can convert prediction confidence intervals to approximate reserves.
\begin{example}[Converting prediction confidence intervals to $\beta$-approximate reserves]
\label{ex:confidenceinterval}
Suppose the platform utilizes some ML model to predict the true value $v_{i,j}$ of bidder $i$ in auction $j$, and produces a confidence interval $(\Hat{v}_{i,j}^{-} , \Hat{v}_{i,j}^{+})\ni v_{i,j}$ with $\Hat{v}_{i,j}^{-},\Hat{v}_{i,j}^{+} > 0$. The platform can then choose personalized reserve $r_{i,j} = \Hat{v}_{i,j}^{-}$, which is $\beta$-approximate for $\beta =\frac{\Hat{v}_{i,j}^{-}}{\Hat{v}_{i,j}^{+}}\in (0,1)$ as $\beta v_{i,j} < \beta \Hat{v}_{i,j}^{+} = r_{i,j} < v_{i,j}$.
\end{example}
% \redsout{Finally, we point out that for autobidders with uniform bid multipliers at least $\beta$, the auction outcome when imposing $\beta$-approximate reserves is the same as that of not having reserves at all. In other words, approximate reserves only change the payment of bidders, but do not alter allocation.} \yuan{This paragraph is a bit confusing and may raise questions. It is better to remove it.}







==> checklist.tex <==
% \section*{Checklist}

% \begin{enumerate}


% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerYes{}
%   \item Did you describe the limitations of your work?
%     \answerYes{}
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerNA{}
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerYes{}
% \end{enumerate}


% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerYes{}
%         \item Did you include complete proofs of all theoretical results?
%     \answerYes{}
% \end{enumerate}


% \item If you ran experiments...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerNA{}
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerNA{}
%         \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerNA{}
%         \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%   \answerNA{}
% \end{enumerate}


% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerNA{}
%   \item Did you mention the license of the assets?
%   \answerNA{}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%   \answerNA{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerNA{}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%   \answerNA{}
% \end{enumerate}


% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerNA{}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerNA{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerNA{}
% \end{enumerate}


% \end{enumerate}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> old1_model.tex <==
6Consider $N$ bidders bidding in $M$ second price auctions (SPA).  Let $v_{i,j}$ be the value of bidder $i$ in auction $j$, and $v_{j}^{+} = \max_{i\in[N]}v_{i,j}$ be the maximum value in auction $j$. Assume for simplicity no pair of bidders have the same value in an auction, i.e. 
$v_{i,j}\neq v_{i',j}$ for any any two bidders $i\neq i'$ and any $j\in[M]$. 
Denote $\mathcal{G}_{i} = \{j\in[M]: v_{i,j} = v_{j}^{+}\}$ as the set of auctions where bidder $i$'s value is the largest among all bidders. Finally, let $\opt_{i} = \sum_{j\in \mathcal{G}_{i}}v_{i,j}$ be the contribution of bidder $i$ to the optimal welfare in the efficient outcome, and similarly define $\opt_{-i} = \sum_{k\neq i}\opt_{k}$ to be the welfare contribution from all bidders other than $i$ in the efficient outcome.

\begin{definition}[$\beta$-approximate reserves]
In an autobidding problem instance with $M$ auctions and $N$ bidders where bidder $i$'s value in auction $j$ is $v_{i,j}$,  we say that reserve prices $\{r_{i,j}\}_{i\in[N],j\in[M]}$ are $\beta$-approximate for some $\beta \in [0,1)$ if $r_{i,j} \in [\beta v_{i,j},v_{i,j})$ for all $i\in[N],j\in[M]$. 
\end{definition}
Note that for autobidders with bid multipliers at least $\beta$, the auction outcome when imposing $\beta$-approximate reserves is the same as that of not having reserves at all. In other words, approximate reserves only change the payment of bidders, but do not alter allocation.


Suppose bidders adopt a uniform bidding strategy with bid multiplier $\alpha_{i} \in \mathcal{A} \subseteq [1,\infty)$, and there exists $0<\boostlb <\boostub$ s.t. bidders are associated with boost values $z_{i,j} \in [\boostlb v_{i,j}, \boostub v_{i,j}]$. 
% Also in each auction, a bidder faces a reserve price $r_{i,j} \in [\beta v_{i,j},v_{i,j})$ for some $\beta \in [0,1)$. We denote an auction instance as $\inst= (\boostlb,\boostub,\beta)$.
 

Let $\bm{x}\in\{0,1\}^{N\times M}$ denote any auction outcome, where $x_{i,j} = 1$ if bidder $i$ won auction $j$ and 0 otherwise. Under any outcome  $\bm{x}$, 
let $\pay_{i,j}(\bm{x})$ be the payment of bidder $i$ in auction $j$, and $\win_{j}(\bm{x})$ be the winner of auction $j$. Further, let $\mathcal{L}_{i}(\bm{x}) = \{j\in \mathcal{G}_{i}: x_{i,j}\neq 1\}$ be the set of auctions in which $i$ has the largest value but did not win, and define $\well_{i}(\bm{x})$, $\loss_{i}(\bm{x})$
as the total welfare and loss of bidder $i$ under outcome $\bm{x}$, respectively, where
\begin{align}
    \well_{i}(\bm{x}) = \sum_{j\in [M]}v_{i,j}x_{i,j},\quad \text{ and }\quad \loss_{i}(\bm{x}) = \sum_{j\in [M]:\well_{i,j}(\bm{x}) < \opt_{i,j}}v_{i,j}(1-x_{i,j})\,.
\end{align}
Finally, we denote $\feas \subseteq \{0,1\}^{N\times M}$
as the set of all feasible outcomes where every bidder's ROI constraint is satisfied. 

For any $\delta \in [0,1]$, we say that an auction instance $\inst$ is $\delta$-fair for bidder $i$ if  
\begin{align}
    \min_{\bm{x}\in \feas}\frac{\well_{i}(\bm{x})}{\opt_{i}}~\geq~ \delta
\end{align}

\begin{proposition}[Connecting loss with fairness]
\label{prop:boundloss}
Assume for bidder $i \in [N]$ and outcome $\bm{x}$ we have $\loss_{i}(\bm{x})\leq B$ for some $B > 0$. Then, $\frac{\well_{i}(\bm{x})}{\opt_{i}}\geq 1- \frac{B}{\opt_{i}}$.
\end{proposition}
\begin{proof}
\begin{align*}
    \opt_{i}-\well_{i}(\bm{x}) = \loss_{i}(\bm{x}) + \sum_{j\in [M]:\well_{i,j}(\bm{x}) > \opt_{i,j}}\left(\opt_{i}-\well_{i}(\bm{x})\right) \leq \loss_{i}(\bm{x}) \leq B\,.
\end{align*}
Rearranging and dividing both sides by $\opt_{i}$ we get $\frac{\well_{i}(\bm{x})}{\opt_{i}}\geq 1- \frac{B}{\opt_{i}}$.
\end{proof}


Our goal is to present a characterization for how model primitives of the auction instance $\inst$ impact overall fairness of bidders.


\begin{theorem}[Fairness lower bound for single bidder]
\label{thm:fairnessbound}
Fix any auction instance $\inst= (\boostlb,\boostub,\beta)$, suppose bidder $i$'s multiplier is $\alpha_{i} > \boostub + 1 -  \boostlb$. Then for any outcome $\bm{x}$ and bidder $i \in [K]$, $\loss_{i}(\bm{x})\leq \frac{1-\beta}{\alpha_{i} + \boostlb - \boostub -1}\opt_{-i}$. Further,
\begin{align}
    \min_{\bm{x}\in \feas}  \frac{\well_{i}(\bm{x})}{\opt_{i}} ~\geq~ 1- \frac{1-\beta}{\alpha_{i} + \boostlb - \boostub -1} \cdot \frac{\opt_{-i}}{\opt_{i}}
\end{align}
\end{theorem}

\begin{proof}
In the following proof, we fix any outcome $\bm{x}$, and omit $\bm{x}$ in the notation for simplicity as the context is clear.
For any bidder $i$ and auction $j \in \mathcal{L}_{i}$ in which bidder $i$ is not the winner but possesses the highest value, we have
\begin{align*}
\begin{aligned}
    \pay_{\win_{j},j} ~\geq~  \left(\alpha_{i}v_{i,j} + z_{i,j} - z_{\win_{j},j}\right)_{+} 
   ~\geq~  \alpha_{i}v_{i,j} + z_{i,j} - z_{\win_{j},j}
    ~\geq~ 
     (\alpha_{i} + \boostlb) v_{i,j} - \boostub v_{\win_{j},j} \,.
    %  \alpha_{i}v_{i,j} + \boostlb v_{i,j} - \boostub v_{\win_{j},j} \\
    % ~=~ &  (\alpha_{i} + \boostlb) v_{i,j} - \boostub v_{\win_{j},j} \,.
    \end{aligned}
\end{align*}
Rearranging, and summing over all auctions in $\mathcal{L}_{i}$, we get
\begin{align}
\begin{aligned}
\label{eq:SPA:loss1}
   \sum_{j\in \mathcal{L}_{i}} v_{i,j} ~\leq~& \frac{\boostub}{\alpha_{i} + \boostlb}\sum_{j\in \mathcal{L}_{i}} v_{\win_{j},j}  + \frac{1}{\alpha_{i} + \boostlb}\sum_{j\in \mathcal{L}_{i}}\pay_{\win_{j},j}
      \end{aligned}
\end{align}


On one hand,
\begin{align*}
\begin{aligned}
    \sum_{j\in \mathcal{L}_{i}}v_{\win_{j},j} +  \sum_{\substack{j\in [M]/\mathcal{G}_{i}\\\win_{j}\neq i}} v_{\win_{j},j}  ~\overset{(a)}{\geq}~& \sum_{j\in \mathcal{L}_{i}}\pay_{\win_{j},j} + \sum_{\substack{j\in [M]/\mathcal{G}_{i}\\\win_{j}\neq i}}\pay_{\win_{j},j}
    ~\overset{(b)}{\geq}~   \sum_{j\in \mathcal{L}_{i}}\pay_{\win_{j},j} + \beta \sum_{\substack{j\in [M]/\mathcal{G}_{i}\\\win_{j}\neq i}}v_{\win_{j},j}\,,
%  ~\overset{(c)}{\geq}~ &  \sum_{j\in \mathcal{L}_{i}}\pay_{\win_{j},j} + \beta \sum_{\substack{j\in [M]/\mathcal{G}_{i}\\\win_{j}\neq i}}v_{\win_{j},j}
   \end{aligned}
\end{align*}
For inequality (a), the LHS denotes the total welfare accumulated in auctions that $i$ did not win (i.e. $\mathcal{L}_{i}\cup \{j \in [M]/\mathcal{G}_{i}:\win_{j}\neq i\}$) by all bidders other than $i$, and the RHS is the total payment in the same set of auctions that are payed by bidders other than $i$. Therefore (a) follows from the ROI constraint, summed over all bidders other than $i$. In (b), we used the fact that for each bidder $k\in[N]$ her payment $p_{k,j}$  in auction $j\in[M]$ is at least her reserve price $r_{k,j}$ in that auction, and by definition of $\beta$-approximate reserves we have  $r_{k,j}\in [\beta v_{k,j}, v_{k,j})$.


Hence by rearranging we get 
\begin{align}
\label{eq:SPA:loss2}
    \sum_{j\in \mathcal{L}_{i}}\pay_{\win_{j},j}~\leq~ (1-\beta)\sum_{\substack{j\in [M]/\mathcal{G}_{i}\\\win_{j}\neq i}}v_{\win_{j},j} + \sum_{j\in \mathcal{L}_{i}}v_{\win_{j},j} ~\overset{(a)}{\leq}~ (1-\beta)\opt_{-i} + \sum_{j\in \mathcal{L}_{i}}v_{\win_{j},j} \,,
\end{align}
where (a) follows from the fact that the accumulated welfare in the set of auctions $\{j \in [M]/\mathcal{G}_{i}:\win_{j}\neq i\}$ (i.e. auctions where $i$ does not have the largest value and also did not win), cannot be greater than the total maximum welfare of all other bidders.

On the other hand, by definition bidder $i$ has the largest value in any auction within the set $\mathcal{L}_{i}\subseteq \mathcal{G}_{i}$, so $v_{k,j} <v_{i,j}$ for any $k\neq j$. Hence,
\begin{align}
\label{eq:SPA:loss3}
    \sum_{j\in \mathcal{L}_{i}} v_{\win_{j},j} ~\leq ~ \sum_{j\in \mathcal{L}_{i}} v_{i,j}\,.
\end{align}
Finally, combining Equations (\ref{eq:SPA:loss1}), (\ref{eq:SPA:loss2}), (\ref{eq:SPA:loss3}) and rearranging we get 
\begin{align}
\begin{aligned}
   & \sum_{j\in \mathcal{L}_{i}} v_{i,j} ~\leq~ \frac{\boostub+1}{\alpha_{i} + \boostlb}\sum_{j\in \mathcal{L}_{i}} v_{\win_{j},j}  + \frac{1-\beta}{\alpha_{i} + \boostlb}\opt_{-i}
    ~\leq~ \frac{\boostub+1}{\alpha_{i} + \boostlb} \sum_{j\in \mathcal{L}_{i}}v_{i,j} + \frac{1-\beta}{\alpha_{i} + \boostlb}\opt_{-i}\\
    \Longleftrightarrow & \sum_{j\in \mathcal{L}_{i}} v_{i,j}~\leq~ \frac{1-\beta}{\alpha_{i} + \boostlb - \boostub -1} \opt_{-i}\,.
\end{aligned}
\end{align}
Recognizing that $\loss_{i}= \sum_{j\in \mathcal{L}_{i}} v_{i,j} $ and applying Proposition \ref{prop:boundloss} yields the desired result.
\end{proof}

\begin{corollary}
For any auction instance $\inst= (\boostlb,\boostub,\beta)$ and $\delta \in (0,1)$, by setting $\beta \geq 1- (1-\delta)\cdot (L+\boostlb - \boostub - 1) \cdot \max_{i\in [K]}\frac{\opt_{i}}{\opt_{-i}}$, the auction instance is $\delta$-fair for all bidders. Here,  $L$  is a multiplier lower bound  for all bidders such that $ L > \boostub - \boostlb+ 1$, and $(1-\delta)\cdot (L+\boostlb - \boostub - 1) \cdot \max_{i\in [K]}\frac{\opt_{i}}{\opt_{-i}} < 1$.
\end{corollary}

\begin{theorem}
adf
\end{theorem}

\begin{proof}
Fix a bidder $i \in [K]$, her bid multiplier $\alpha_{i}$, and any outcome $\bm{x}=(\bm{x}_{1} ... \bm{x}_{M})$ where $\bm{x}_{j} \in \{0,1\}^{N\times \numslot_{j}}$ is the outcome vector in auction $j$.

Denote $\ell_{k,j}$, $\ell_{k,j}^{\opt}$ to be the position of bidder $k\in[N]$ in auction $j\in [M]$ under outcome $\bm{x}$ and the efficient outcome, respectively. Consider an auction $j$ where $\ell_{i,j} > \ell_{i,j}^{\opt}$, i.e. in auction $j$, bidder $i$ acquires a position bellow that of her position in the efficient outcome. Then there exists a bidder $\kappa_{j}$ such that 
\begin{align}
\label{eq:VCG:badbidder}
    v_{\kappa_{j},j} < v_{i,j},  \quad \text{ and } ~\ell_{\kappa_{j},j} \leq \ell_{i,j}^{\opt} <  \ell_{i,j}
\end{align}
Consider the payment of bidder $\kappa_{j}$:
\begin{align}
\begin{aligned}
\label{eq:VCG:badbidder1}
    p_{\kappa_{j},j}~\geq~& \sum_{\ell = \ell_{\kappa_{j},j}}^{\numslot_{j}}\left(\mu(\ell) - \mu(\ell+1)\right)\Hat{b}_{\ell+1}\\
    ~\overset{(a)}{=}~& \sum_{\ell = \ell_{\kappa_{j},j}}^{\ell_{i,j}^{\opt}-1}\left(\mu(\ell) - \mu(\ell+1)\right)\Hat{b}_{\ell+1}+\sum_{\ell = \ell_{i,j}^{\opt}}^{\ell_{i,j}-1}\left(\mu(\ell) - \mu(\ell+1)\right)\Hat{b}_{\ell+1} +  p_{i,j}\\
    %  ~\geq~& \sum_{\ell = \ell_{\kappa_{j},j}}^{\ell_{i,j}-1}\left(\mu(\ell) - \mu(\ell+1)\right)\Hat{b}_{\ell+1} + \alpha_{i}\left(\mu(\ell_{i,j}^{\opt}) - \mu(\ell_{i,j})\right) v_{i,j} + \beta \cdot  \mu(\ell_{i,j})v_{i,j}\\
     ~\overset{(b)}{\geq}~&  \left(\mu(\ell_{\kappa_{j},j}) - \mu(\ell_{i,j})\right)v_{i,j} + \alpha_{i}\left(\mu(\ell_{i,j}^{\opt}) - \mu(\ell_{i,j})\right) v_{i,j} + \beta \cdot  \mu(\ell_{i,j})v_{i,j}\\
      ~=~&  \mu(\ell_{\kappa_{j},j}) v_{i,j} + \alpha_{i}\left(\mu(\ell_{i,j}^{\opt}) - \mu(\ell_{i,j})\right) v_{i,j} - (1- \beta) \cdot  \mu(\ell_{i,j})v_{i,j}\\
    \end{aligned}
\end{align}

On the other hand, we have
\begin{align*}
      & p_{\kappa_{j},j} + \sum_{j'\neq j}  p_{\kappa_{j},j'} \leq \mu(\ell_{\kappa_{j},j})v_{\kappa_{j},j} + \sum_{j'\neq j}  \mu(\ell_{\kappa_{j},j'})v_{\kappa_{j},j'} \overset{(a)}{<} \mu(\ell_{\kappa_{j},j})v_{i,j} + \sum_{j'\neq j}  \mu(\ell_{\kappa_{j},j'})v_{\kappa_{j},j'}\\
      &  p_{\kappa_{j},j'}\geq \beta\cdot \mu(\ell_{\kappa_{j},j'})v_{\kappa_{j},j'} \quad \forall j'\in[M]\,,
\end{align*}
where the first inequality follows from bidder $\kappa_{j}$'s ROI constraint, and in (a) we used Equation (\ref{eq:VCG:badbidder}); the second  inequality follows from the fact that any winning bidder's payment must be greater than her $\beta$-approximate reserves. Combining the above inequalities and rearranging we get
\begin{align}
\label{eq:VCG:badbidder2}
    p_{\kappa_{j},j} < \mu(\ell_{\kappa_{j},j})v_{i,j} + (1-\beta)\cdot \sum_{j'\neq j}  \mu(\ell_{\kappa_{j},j'})v_{\kappa_{j},j'}\,,
\end{align}
Combining Equations (\ref{eq:VCG:badbidder1}) and (\ref{eq:VCG:badbidder2}), we get
\begin{align}
  \alpha_{i}\left(\mu(\ell_{i,j}^{\opt}) - \mu(\ell_{i,j})\right) v_{i,j} < (1- \beta) \cdot  \mu(\ell_{i,j})v_{i,j} + (1-\beta)\cdot \sum_{j'\neq j}  \mu(\ell_{\kappa_{j},j'})v_{\kappa_{j},j'} 
\end{align}
Summing the above over all $j \in \mathcal{L}_{i} = \{j\in[M]: \ell_{i,j} > \ell_{i,j}^{\opt}\}$, we have
\begin{align}
\begin{aligned}
  \sum_{j \in \mathcal{L}_{i}}\left(\mu(\ell_{i,j}^{\opt}) - \mu(\ell_{i,j})\right) v_{i,j} ~<~ & \frac{1-\beta}{\alpha_{i}}\left(\sum_{j \in \mathcal{L}_{i}}\mu(\ell_{i,j})v_{i,j} + \sum_{j \in \mathcal{L}_{i}} \sum_{j'\neq j}  \mu(\ell_{\kappa_{j},j'})v_{\kappa_{j},j'} \right)\\
  ~\leq~ &  \frac{1-\beta}{\alpha_{i}}\well(\bm{x}) \leq \frac{1-\beta}{\alpha_{i}}\opt \,.
  \end{aligned}
\end{align}

\end{proof}



In the following theorem, we present a problem instance where the fairness lower bound in Theorem \ref{thm:fairnessbound} is tight.
\begin{theorem}[Matching fairness upper bound]
Consider 2 bidders competing in 3 SPA auctions whose values are indicated in the following table. 
\renewcommand{\arraystretch}{2}
\begin{center}
\begin{tabular}{|c | c c c | c|} 
 \hline
  & Auction 1 & Auction 2 & Auction 3 & Uniform boost coef.\\
 \hline\hline
 bidder 1 & $\gamma$ & $v$ & 0 & $\boostlb$\\ 
 \hline
 bidder 2 & 0  & $v-\epsilon$ & $\gamma + \frac{\boostub+1}{1-\beta}\cdot \epsilon$ & $\boostub$  \\
 \hline
\end{tabular}
\end{center}
Here, fix bidder 1's multiplier to be some $\alpha_{1} > \boostub+1-\boostlb$, and consider $v = \frac{1-\beta}{\alpha_{1}+\boostlb - \boostub-1} \cdot \gamma$. Also, consider uniform boosts with boost coefficients $\boostlb$, $\boostub$ for bidder 1 and 2, respectively, i.e. $z_{1,j} = \boostlb v_{1,j}$ and  $z_{2,j} = \boostub v_{2,j}$ for all auctions $j = 1,2,3$. The reserve prices are set to be $r_{i,j} = \beta v_{i,j}$ for some $\beta \in (0, \min\{1,\alpha_{1} + \boostlb - \boostub\})$. Then, we have
\begin{align}
    \min_{\bm{x}\in \feas}  \frac{\well_{1}(\bm{x})}{\opt_{1}} ~=~ 1- \frac{1-\beta}{\alpha_{i} + \boostlb - \boostub -1} \cdot \frac{\opt_{-i} - \frac{\boostub+1}{\beta}\cdot \epsilon}{\opt_{i}}
\end{align}
Taking $\epsilon \to 0$ yields the desired matching fairness upper bound.
\end{theorem}

\begin{proof}
Note that in any feasible outcome, bidder 1 must win auction 1, and bidder 2 must win auction 3.  Hence for auction 2, we only need to consider the following outcome:
% For auction 2, there are only 2 possible outcomes, namely bidder 1 wins or bidder 2 wins.

% \textbf{Bidder 1 wins auction 2, and suffers no welfare loss.} This outcome can be achieved by having $\alpha_{2}$ such that $(\alpha_{2}+ \boostub) (v-\epsilon) < (\alpha_{1}+ \boostlb)v$. Bidder 1 accumulates value $\gamma+v = \opt_{1}$, and pays $\beta \gamma + \max\{\beta v,(\alpha_{2}+ \boostub) (v-\epsilon) - \boostlb v\}$, which is obviously less than $\opt_{1}$ since $\beta < 1$, so bidder 1's ROI constraint is satisfied. It is also trivial that bidder 2's ROI constraint is satisfied. 

\textbf{Bidder 1 loses auction 2, and suffers welfare loss $v$.} This outcome can be achieved by setting $\alpha_{2}$ such that $(\alpha_{2}+ \boostub) (v-\epsilon) > (\alpha_{1}+ \boostlb)v$. Bidder 2 accumulates value $v + \gamma + \left( \frac{\boostub+1}{1-\beta}-1\right)\epsilon$. Her payment for auction 2 is $\max\{(\alpha_{1} + \boostlb)v -  \boostub(v-\epsilon),\beta(v-\epsilon)\}$, and for auction 3 is $\beta\left(\gamma + \frac{\boostub+1}{\beta}\cdot \epsilon\right)$. The following shows that her ROI constraint is satisfied:
\begin{align*}
    & v + \gamma + \left( \frac{\boostub+1}{1-\beta}-1\right)\epsilon - \max\{(\alpha_{1} + \boostlb)v -  \boostub(v-\epsilon),\beta(v-\epsilon)\} - \beta\left(\gamma + \frac{\boostub+1}{1-\beta}\cdot \epsilon\right)\\
    ~\overset{(a)}{=}~ & v + \gamma + \left( \frac{\boostub+1}{1-\beta}-1\right)\epsilon - (\alpha_{1} + \boostlb)v +  \boostub(v-\epsilon) - \beta\left(\gamma + \frac{\boostub+1}{1-\beta}\cdot \epsilon\right)\\
     ~=~ & \left(\boostub + 1 - \alpha_{1} - \boostlb\right)v + (1-\beta)\gamma + \left(\frac{\boostub+1}{1-\beta}-1 - \boostub - \beta\cdot \frac{\boostub+1}{1-\beta}\right)\epsilon\\
      ~=~ & 0\,,
\end{align*}
where in (a) we used the fact $\beta < \alpha_{1} + \boostlb - \boostub $, so that 
$$ \beta(v-\epsilon)< \beta v < (\alpha_{1} + \boostlb - \boostub) v < (\alpha_{1} + \boostlb)v -  \boostub(v-\epsilon)\,.$$
In the final equality we used the definition that $v = \frac{1-\beta}{\alpha_{1}+\boostlb - \boostub-1} \cdot \gamma$. On the other hand, bidder 1's ROI constraint is apparently satisfied. 

Under this outcome, we have 
\begin{align*}
    \frac{\well_{1}}{OPT_{1}} = 1- \frac{v}{OPT_{1}}= 1- \frac{1-\beta}{\alpha_{i} + \boostlb - \boostub -1} \cdot \frac{\gamma}{\opt_{i}} =  1- \frac{1-\beta}{\alpha_{i} + \boostlb - \boostub -1} \cdot \frac{\opt_{-i} - \frac{\boostub+1}{\beta}\cdot \epsilon}{\opt_{i}}
\end{align*}
\end{proof}




\section{Impossibility Result: VCG with reserve is the fairest}
Can we improve individual fairness guarantees via other auction formats? The answer is negative. We show that for any auction that is anonymous and truthful, there exists an autobidding instance consisting of multiple auctions and bidders where there must be a bidder that will incur a welfare loss at least.  


\begin{definition}[Anonymous auction]
Consider any auction mechanism $\mathcal{M}$ whose (possibly random) allocation $\mathcal{X}:\R^{N}\to \R^{N}$ satisfies $\sum_{i\in[N]}\mathcal{X}_{i}(\bm{b}) = 1$ for any number of bidders $N$ and bid profile $\bm{b} \in \R_{\geq 0}^{N}/\{\bm{0}\}$. Then we say $\mathcal{M}$ is anonymous if the outcome for a permutation of any bid profile $\bm{b}$ is the permutation of the outcome for $\bm{b}$, i.e. for any permutation $\sigma: [N]\to [N]$, then $\left[\mathcal{X}(b_{\sigma(1), \dots \sigma(N)})\right]_{i} = \left[\mathcal{X}(\bm{b})\right]_{\sigma(i)} $ for any $i \in [N]$.
\end{definition}
As an example, the second price auction with $\beta$-approximate reserves is anonymous.

\begin{lemma}
\label{lem:winprobub}
In an anonymous and truthful auction for a single item with $N$ bidders, the bidder who submits the lowest bid wins the item with probability at most $\frac{1}{N}$.
\end{lemma}

\begin{definition}[Monopolist purchase probability and bid threshold]
\label{def:monop}
For any anonymous and truthful auction $\mathcal{M}$, consider the setting with a single bidder. Let $b > 0$ be the submitted bid, and define 
\begin{align}
    \pi_{\mathcal{M}} = \lim_{b\to \infty}\prob(\text{bidder wins item with bid $b$})\,,
\end{align}
where the limit exists because in a truthful auction, $\prob(\text{bidder wins item with bid $b$})$ increases in $b$. Assume this max probability is reached at some bid threshold $Q_{\mathcal{M}}$, i.e.
\begin{align}
   Q_{\mathcal{M}} = \min\left\{b>0: \prob(\text{bidder wins item with bid $b$}) =  \pi_{\mathcal{M}}\right\} \,.
\end{align}
\end{definition}

\begin{lemma}[\cite{mehta2022auction}]
For any anonymous and truthful auction $\mathcal{M}$ with monopolist purchase probability $ \pi_{\mathcal{M}}$ and bid threshold $ Q_{\mathcal{M}}$, the expected cost for a single bidder for winning the item is at most $\pi_{\mathcal{M}} \cdot Q_{\mathcal{M}}$.
\end{lemma}

\begin{theorem}
For any auction $\mathcal{M}$ that is anonymous and truthful, consider an autobidding problem instance w.r.t.  $\mathcal{M}$ with $M = 2K+1$ auctions and $N = K+1$ bidders. Fix bidder 0's bid multiplier to be $\alpha_{0}$ and some $\beta\in [0,1)$. Consider the bidder values $\{v_{i,j}\}_{i\in[N],j\in[M]}$, and assume in each auction $j$ we impost a single reserve $r_{j}$, both given in the followin table.
\renewcommand{\arraystretch}{2}
\begin{center}
\begin{tabular}{|c | c c c c c c c c c|} 
 \hline
  & $A_{1}$ & $A_{2}$ & \dots  &   $A_{K}$  & $A_{K+1}$ & $A_{K+2}$ & \dots & $A_{2K}$ &  $A_{2K+1}$\\
 \hline\hline
 $B_{0}$ & $v$ & $v$ & \dots & $v$ & 0 & 0 & \dots & 0  & $X$\\ 
 \hline
$B_{1}$  & $\frac{\alpha_{0}v+\epsilon}{\rho}$ & $\frac{\alpha_{0}v+2\epsilon}{\rho}$  & \dots &  $\frac{\alpha_{0}v+K\epsilon}{\rho}$ & $\gamma$  & 0 &  \dots & 0 & 0\\
  \hline
 $B_{2}$  & $\frac{\alpha_{0}v+2\epsilon}{\rho}$ & $\frac{\alpha_{0}v+3\epsilon}{\rho}$  & \dots &  $\frac{\alpha_{0}v+\epsilon}{\rho}$ & 0 &  $\gamma$ & \dots &  0 & 0  \\
 \hline
 \vdots & \vdots &  \vdots  &  &   \vdots  &  \vdots & \vdots & & \vdots & \vdots \\
  \hline
   $B_{K}$  & $\frac{\alpha_{0}v+K\epsilon}{\rho}$ & $\frac{\alpha_{0}v+\epsilon}{\rho}$  & \dots &  $\frac{\alpha_{0}v+(K-1)\epsilon}{\rho}$ & 0  & 0  & \dots & $\gamma$ & 0\\
   \hline
   \hline
   Reserve & $\beta v$ & $\beta v$  & \dots & $\beta v$  & $\beta \gamma$ &  $\beta \gamma$ & \dots &  $\beta \gamma$ & $\beta X$\\
   \hline
\end{tabular}
\end{center}
In the table, we let $\gamma > \frac{Q_{\mathcal{M}}}{\beta} > Q_{\mathcal{M}}$, $\epsilon = O(1/K^{3})$ and $v = \frac{1-\beta}{\alpha_{0}-1}\cdot \pi_{\mathcal{M}}\cdot \gamma$. Let $\rho,X$ and a large enough $K$ satisfy the following:
\begin{align}
\begin{aligned}
\label{eq:imposs:params}
%   & \gamma \geq \max\left\{\frac{1}{(1-\beta)\pi_{\mathcal{M}}}\left( \frac{(1-\beta)\alpha_{0}}{\alpha_{0}-1} + \frac{(K+1)K}{2}\epsilon\right),\frac{Q_{\mathcal{M}}}{\beta} \right\}\\ 
   & \alpha_{0}<\rho <\frac{\alpha_{0}}{\beta} ~\text{s.t.}~\frac{\alpha_{0}v+K\epsilon}{\rho} < v,\quad \text{ and } X > \max\left\{\frac{Q_{\mathcal{M}}}{\alpha_{0}}, \frac{\alpha_{0}v}{\pi_{\mathcal{M}}}\right\}\,.
  \end{aligned}
\end{align}
 Then, when bidders 1, ... K all adopt the bid multiplier $\rho$, bidder $0$'s fairness guarantee is at most $1-\frac{1-\beta}{\alpha_{0}-1}\cdot \frac{\opt_{-0}}{\opt_{0}}$.
\end{theorem}
\begin{remark}
Note that in each auction $j\in[M]$, the reserve price $r_{j} \geq \beta v_{i,j}$ for any $i \in [N]$, so these reserve prices are $\beta$-approximate. 
\end{remark}

\begin{proof}


\begin{align}
\begin{aligned}
     \loss_{0} ~\geq~ &  v\sum_{j\in [K]}\prob(\text{bidder 0 loses auction $j$})~=~  v\sum_{j\in [K]}\left(1-\prob(\text{bidder 0 wins auction $j$})\right)\\
    ~\overset{(a)}{\geq}~ & v \cdot \frac{K^{2}}{K +1} = \frac{1-\beta}{\alpha_{0}-1}\cdot \gamma \cdot \pi_{\mathcal{M}} \cdot \frac{K^{2}}{K +1} =  \frac{1-\beta}{\alpha_{0}-1} \cdot \E_{\mathcal{M}}\left[\opt_{-0}\right] \cdot \frac{K}{K+1}\,.
    % > \frac{1-\beta}{\alpha_{0}-1}\gamma (K-1) = \frac{1-\beta}{\alpha_{0}-1}\opt_{-0}
    \end{aligned}
\end{align}
Here (a) holds because bidder 0 bids $\alpha_{0}v$ for any auction in 1,2...K, which is strictly less than all other bidders' bids as they all adopt  multipliers $\rho$ in these auctions, so from Lemma \ref{lem:winprobub}, we have $\prob(\text{bidder 0 wins auction $j$})\leq \frac{1}{K+1}$.

Therefore we have 
\begin{align}
    \lim_{K\to \infty}\frac{\loss_{0}}{\E_{\mathcal{M}}\left[\opt_{-0}\right]} \geq \frac{1-\beta}{\alpha_{0}-1}\cdot  \frac{K}{K+1} =  \frac{1-\beta}{\alpha_{0}-1}\,.
\end{align}

Now it only remains to show that the multiplies $(\alpha_{0}, \rho, \dots \rho) \in (1,\infty)^{K+1}$ yields a feasible outcome, i.e. the ROI constraints of each bidder is satisfied in expectation. Let $V_{i,j}$ and $C_{i,j}$  be the expected value and cost of bidder $i$ in auction $A_{j}$, respectively.

\textbf{1. Showing bidder $0$'s ROI constraint is satisfied}.
We show by the following: bidder 0 only incurs a non-zero expected cost in auctions $A_{1}\dots A_{K}$ and $A_{2K+1}$, and we will show that the expected value $V_{0,2K+1}$ is lower bounded by the expected costs $C_{0,2K+1} + \sum_{j\in[K]}C_{0,j}$.

Since $\alpha_{0}X  > Q_{\mathcal{M}}$, the definition of the monopolist purchasing probability in Definition \ref{def:monop} implies that  bidder 0 acquires an expected value from  auction $A_{2K+1}$ of $V_{0,2K+1} = \pi_{\mathcal{M}}X$. Further,  since bidder 0 is submits the lowest bids in auctions $A_{1} \dots A_{K}$ under bid multiplier profile $(\alpha_{0},\rho \dots \rho)\in (0,\infty)^{K+1}$,  from Lemma \ref{lem:winprobub}, we have $\prob(\text{bidder 0 wins auction $j$})\leq \frac{1}{K+1}$ for all $j \in [K]$. Since the payment of a bidder in an auction is at most her submitted bid, we know that $\sum_{j \in [K]}C_{0,j}\leq  K\cdot \frac{\alpha_{0}v}{K+1} < \pi_{\mathcal{M}}X = V_{0,2K+1}$, where the inequality follows from the definition of $X$ in Equation (\ref{eq:imposs:params}) such that $X > \max\left\{\frac{Q_{\mathcal{M}}}{\alpha_{0}}, \frac{\alpha_{0}v}{\pi_{\mathcal{M}}}\right\}$. This implies bidder 0's ROI constraint is satisfied.

\textbf{2. Showing bidder $i$'s ROI constraint is satisfied for any $i = 1,2 \dots K$}. We show by the following: bidder $i$ only incurs a non-zero expected cost in auctions $A_{1}\dots A_{K}$ and $A_{K+i}$, and we will show that the expected values $ \sum_{k\in [K+1]}V_{i,j}$ is lower bounded by the expected costs $C_{i,K+i} + \sum_{j\in[K]}C_{i,j}$.

\begin{itemize}
 
    \item \textbf{Calculate cost $C_{i,K+i}$: } For auction $A_{K+i}$, bidder $i$'s bid is $\rho\gamma > \gamma > Q_{\mathcal{M}}$ from the definition of $\gamma$, so by Definition \ref{def:monop}, the probability of $i$ winning the item in auction $A_{K+i}$ is $\pi_{\mathcal{M}}$, and the expected cost is
    \begin{align}
    \label{eq:imposs:costub}
     C_{i,K+i} \leq \pi_{\mathcal{M}}\cdot \max\left\{r, Q_{\mathcal{M}}  \right\} \leq \pi_{\mathcal{M}}\cdot\beta \gamma\,,
     \end{align}
     where the final inequality follows from the definition $r = \beta\cdot \min_{i\in[N],j\in[M]}v_{i,j}  $
     
     \item \textbf{Upper bound costs $\sum_{j\in[K]}C_{i,j}$: }  
             For auctions $[K] = 1\dots K$,  bidder $i$'s total expected cost can be bounded as
        \begin{align}
        \begin{aligned}
        \label{eq:imposs:costub2}
           \sum_{j\in[K]} C_{i,j} ~\leq~ & \rho \sum_{j\in[K]} v_{i,j} \prob\left(\text{bidder $i$ wins auction $A_{j}$}\right)\\
           ~\leq~ & \alpha_{0}v \sum_{j \in [K]}\prob\left(\text{bidder $i$ wins auction  $A_{j}$}\right) + \frac{(K+1)K}{2}\epsilon \\
            ~\overset{(a)}{\leq}~ & \alpha_{0}v+ \frac{(K+1)K}{2}\epsilon \\
           \end{aligned}
        \end{align}
        In (a) we used the fact that $ \sum_{j \in [K]}\prob\left(\text{bidder $i$ wins auction  $A_{j}$}\right)\leq 1 $ due to the following:
        
        Consider the bid profile $\bm{b} = (\alpha_{0}v, \alpha_{0}v+\epsilon, \alpha_{0}v+2\epsilon \dots \alpha_{0}v+ K\epsilon)\in \R_{+}^{K+1}$. By anonymity of auction $\mathcal{M}$, there exists probabilities $\bm{q}(\bm{b})=(q_{0}(\bm{b}),q_{1}(\bm{b}) \dots q_{K}(\bm{b})) \in [0,1]^{K+1}$ where $$q_{k}(\bm{b}) = \prob(\text{bid value $b_{k}$ wins auction $\mathcal{M}$ given competing bids $\bm{b}_{-k}$}) \quad \text{ and } \sum_{k=0}^{K}q_{k}(\bm{b})= 1.$$
        By recognizing $\bm{b}$ is exactly the set of bids in each auction $A_{1} \dots A_{K}$ under bid multipliers $(\alpha_{0},\rho,\dots \rho)\in (1,\infty)^{K+1}$, we know that
        \begin{align}
        \label{eq:imposs:competewinbound}
            \sum_{j \in [K]}\prob\left(\text{bidder $i$ wins auction $j$}\right) =  \sum_{k = 1}^{K} q_{k}(\bm{b}) = 1-  q_{0}(\bm{b})\leq 1
        \end{align}
       
     \item \textbf{Calculate $V_{i,K+i}$: }
        Considering auction $A_{K+i}$, bidder $i$ is the only bidder, and since $\rho \gamma >\gamma > Q_{\mathcal{M}}$, the definition of the monopolist purchasing probability in Definition \ref{def:monop} implies that  bidder $i$'s acquires an expected value from this auction of 
    \begin{align}
    \label{eq:imposs:vallb}
        V_{i,K+i} = \pi_{\mathcal{M}}\cdot \gamma\,.
    \end{align} 
    
    \item \textbf{Lower bound $\sum_{k\in [K]}V_{i,j}$: }
    
    \begin{align}
    \label{eq:imposs:vallb2}
        \sum_{k\in [K]}V_{i,j} \geq \frac{\alpha_{0}v}{\rho}\sum_{j\in [K]}\prob\left(\text{bidder $i$ wins auction $j$}\right) \overset{(a)}{=} \frac{\alpha_{0}v}{\rho} \left(1-q_{0}(\bm{b})\right) \overset{(b)}{\geq} \frac{\alpha_{0}v}{\rho} \cdot \frac{K}{K+1}
    \end{align}
    where (a) follows from Equation (\ref{eq:imposs:competewinbound}) where we
    upper bounded $\sum_{j\in[K]}C_{i,j}$ and recall $\bm{b}= (\alpha_{0}v, \alpha_{0}v+\epsilon, \alpha_{0}v+2\epsilon \dots \alpha_{0}v+ K\epsilon)\in \R_{+}^{K+1}$; (b)
    follows from Lemma \ref{lem:winprobub} s.t. $q_{0}(\bm{b})\leq \frac{1}{K+1}$. This is 
    because $q_{0}(\bm{b})$ is the probability of winning with bid value $\alpha_{0}v$ when the other bids $(\alpha_{0}v+\epsilon, \alpha_{0}v+2\epsilon \dots \alpha_{0}v+ K\epsilon)\in \R_{+}^{K}$ are all greater than $\alpha_{0}v$.
\end{itemize}

Finally, combining Equations  (\ref{eq:imposs:costub}),(\ref{eq:imposs:costub2}),(\ref{eq:imposs:vallb}) and (\ref{eq:imposs:vallb2}), we get
\begin{align*}
     & \sum_{j\in[K]}V_{i,j}  + V_{i,K+i} -  \left(\sum_{j\in[K]}C_{i,j} C_{i,K+i}\right) \\   
     ~\geq~ & \pi_{\mathcal{M}}\cdot \gamma  +\frac{\alpha_{0}v}{\rho} \cdot \frac{K}{K+1} - \left(\pi_{\mathcal{M}}\cdot\beta \gamma + \alpha_{0}v +  \frac{(K+1)K}{2}\epsilon\right)\\
     ~=~ &  \pi_{\mathcal{M}}\cdot (1-\beta) \gamma + \left(\alpha_{0}- \frac{\alpha_{0}}{\rho}\cdot \frac{K}{K+1} \right) v -  \frac{(K+1)K}{2}\epsilon\\
     ~=~ &  (\alpha_{0}-1)v + \left(\alpha_{0}- \frac{\alpha_{0}}{\rho}\cdot \frac{K}{K+1} \right) v -  \frac{(K+1)K}{2}\epsilon\,,
\end{align*}
where the final equality follows from the definition $v = \frac{1-\beta}{\alpha_{0}-1}\cdot \pi_{\mathcal{M}}\cdot \gamma$.

Finally, by taking $\rho \to \alpha_{0}$ and $K\to\infty$, and utilizing $\epsilon = O(1/K^{3})$ we have
\begin{align*}
& \lim_{\rho \to \alpha_{0}} \lim_{K\to\infty}\sum_{j\in[K]}V_{i,j}  + V_{i,K+i} -  \left(\sum_{j\in[K]}C_{i,j} C_{i,K+i}\right)~\geq~ 0 \,.
\end{align*}
This shows that bidder $i$'s ROI constraint is satisfied.

\end{proof}
